Relaxed Marginal Consistency for Differentially Private Query Answering

Many differentially private algorithms for answering database queries involve a step that reconstructs a discrete data distribution from noisy measurements. This provides consistent query answers and reduces error, but often requires space that grows exponentially with dimension. Private-PGM is a recent approach that uses graphical models to represent the data distribution, with complexity proportional to that of exact marginal inference in a graphical model with structure determined by the co-occurrence of variables in the noisy measurements. Private-PGM is highly scalable for sparse measurements, but may fail to run in high dimensions with dense measurements. We overcome the main scalability limitation of Private-PGM through a principled approach that relaxes consistency constraints in the estimation objective. Our new approach works with many existing private query answering algorithms and improves scalability or accuracy with no privacy cost.

==> approach_dan_bak.tex <==
\section{Our Approach}

In this section we describe our approach to overcome the main scalability limitations of \pgm, by introducing suitable approximations and new algorithmic techniques.  Our innovations allow us to scale significantly better than \pgm with respect to the size of $\C$. A high-level idea is to use approximate marginal inference in the \prox algorithm, but doing so naively makes it unclear what, if any, formal problem is being solved. We will develop a principled approach that uses approximate inference to \emph{exactly} solve a relaxed optimization problem.

\subsection{Region Graph}

\begin{figure}
  \begin{subfigure}[b]{0.19\textwidth}
    \centering\includegraphics[width=\textwidth]{fig/ex_clique}
    \caption{\label{fig:junction} Junction Tree}
  \end{subfigure}%
  \hspace{2em}
  \begin{subfigure}[b]{0.38\textwidth}
    \centering\includegraphics[width=\textwidth]{fig/ex_factor}
    \caption{\label{fig:factor} Factor Graph}
  \end{subfigure}%
  \hspace{2em}
  \begin{subfigure}[b]{0.38\textwidth}
    \centering\includegraphics[width=\textwidth]{fig/ex_region}
    \caption{\label{fig:region} Saturated Region Graph}
  \end{subfigure}%
\caption{\label{fig:regions} Comparison of different region graph structures defined over a domain with attributes $\set{A,B,C,D,E}$ that support the cliques $\C = \set{\set{A,B,C}, \set{A,D}, \set{B,C,D}, \set{D,E}}$.}
\end{figure}

Central to our approach is the notion of a \emph{region graph}.  A region graph is a data structure that (1) encodes constraints between subsets of attributes in a natural graphical format and (2) facilitates message passing algorithms for approximate marginal inference.


\begin{definition}[Region Graph]
A region graph $G = (\V, \E)$ is a directed graph where every vertex $r \in \V$ is an attribute clique and for any edge $r \rightarrow s \in \E$ we have that $ r \supseteq s $. We say that $G$ supports a clique set $\C$ if for every clique $r \in \C$, there exists some $r' \in \V$ such that $r \subseteq r'$.
\end{definition}
For any region graph, there is a corresponding set of constraints that characterize the \emph{local polytope} of internally consistent \emph{pseudo-marginals}, defined below.  

\begin{definition}[Local Polytope]
The local polytope of pseudo-marginals associated with a region graph $G$ is:
\begin{equation} \label{eq:localpolytope}
\L(G) =
  \left\{ \btau \geq 0
  \;\middle\vert\;
  \begin{array}{@{}l@{}l@{}}
  %\sum_{\x_r} \btau_r(\x_r) = 1 & \forall r \in \V \\
  %\sum_{\x_r \setminus \x_t} \btau_r(\x_r) = \btau_t(\x_t) \quad\quad & \forall r \rightarrow t \in \E\\
  \mathbf{1}^{\top} \btau_r = 1 & \forall r \in \V \\
  P_{r \rightarrow s} \btau_r = \btau_s \quad \quad & \forall r \rightarrow s \in \E \\
  \end{array}
  \right\}.
\end{equation}
\end{definition}

The general idea is to relax problems involving the intractable marginal polytope to use the local polytope instead, since $\M(\V) \subseteq \L(G)$ and $\L(G)$ is straightforward to representat using the linear constraints in Eq.~\eqref{eq:localpolytope}.  We use the notation $\btau$ in place of $\btau$ to emphasize that $\btau$ is not necessarily a valid marginal vector, even though we will generally treat it as such.  This notational choice is standard in the graphical models literature \cite{wainwright2008graphical}.

The nodes and edges in the region graph dictate which constraints we expect to hold among pseudo-marginals.  As discussed  below, region graphs can encode junction trees and factor graphs as special cases.  
%
For example, \cref{fig:regions} shows three different region graphs that support $\C = \set{\set{A,B,C}, \set{A,D}, \set{B,C,D}, \set{D,E}}$.  At one extreme is the \textbf{Junction Tree}, shown in \cref{fig:junction}, which is obtained by merging cliques \set{A,B,C}, \set{A,D}, and \set{B,C,D} into a super-clique $\set{A,B,C,D}$. This region graph structure exactly encodes the marginal polytope, that is, $\L(G) \equiv \M(\V)$. Ordinary belief propagation in this graph corresponds to exact marginal inference.  At the other end of the extreme is the \textbf{Factor Graph}, shown in \cref{fig:factor}.  This graph contains one vertex for every clique $r \in \C$, plus additional vertices for the singleton cliques.  It encodes constraints that all cliques must agree on common one-way marginals. For example, $\btau_{ABC}$ and $\btau_{BCD}$ must agree on the shared one-way marginals $\btau_B$ and $\btau_C$, but not necessarily on the shared two-way marginal $\btau_{BC}$.  A natural middle ground is the fully \textbf{Saturated Region Graph}, shown in \cref{fig:region}.  This graph includes every clique $r \in \C$ as a vertex, and includes additional vertices to capture intersections between those cliques.  Unlike the factor graph, this graph does require that $\btau_{ABC}$ is consistent with $\btau_{BCD}$ with respect to the $\btau_{BC}$ marginal.  Unlike the junction tree, this graph does not require forming super-cliques whose size grow quickly with $|\C|$.  For more details about the concepts above, please refer to \cite{koller2009probabilistic}.
%\ds{Give citations for facts and background concepts in this pargraph that are not fully explained or supported, e.g., junction tree, saturated region graph. A blanket citation might work, but targeted could be better.} \ry{agree targeted is nice, but I think I would just cite Koller and Friedman for all of these.}


The methods we describe in this paper apply for any region graph that supports $\C$.
By default, we simply use the fully saturated region graph, which can easily be constructed given the cliques $\C$ \cite{koller2009probabilistic}.

\begin{definition}[Saturated Region Graph]
Given a set of cliques $\C$, the associated saturated region graph is constructed as follows:\ry{TODO}
\begin{enumerate}
\item $\C \subseteq \V$
\item $\V$ is closed under intersection
\item Whenever $r \supseteq s $ and there is no $t$ such that $ r \supseteq t \supseteq s$, there is an edge $r \rightarrow s$.  
\item cliques in $\C$ do not have parents (or if they do, parents are also in $\C$)
\end{enumerate}
\end{definition}

%% \ds{Orphaned:} For a graphical model $\p_\btheta$ on clique set $\C$ and a region graph that supports $\C$, the goal is to estimate the marginal distributions associated with each vertex in the graph, i.e., $\btau = (\btau_r)_{r \in V}$. Since $G$ supports $\C$, we can easily compute $(\btau_r)_{r \in \C}$ from $(\btau_r)_{r \in V}$ via marginalization, so this solves our original inference goal of estimating $\M_\C \p_\btheta$. Additionally, we can optimize any function over $\M(\C)$ by optimizing an equivalent function over $M(\V)$.\footnote{Let $P$ be the marginalization operation to compute $\btau_r$ from $\btau_{r'}$ for some $r' \in \V$ for each $r \in \C$. $P$ is linear and maps $\M(\V)$ onto $\M(\C$), therefore $\min_{\btau \in \M(\C)} L(\btau) = \min_{\btau' \in \M(\V)}L'(\btau')$ for $L'(\btau') = L(P\btau')$.}

\subsection{Estimation: Finding an Approximate Data Distribution Representation}

We begin by introducing a very natural relaxation of the problem we seek to solve.

\begin{problem}[Convex Optimization over the Local Polytope] \label{prob:convex}
Given a region graph $G$ and a convex loss function $L(\btau)$ where $\btau = (\btau_r)_{r \in V}$, solve:
%
$$ \hat{\btau} = \argmin_{\btau \in \L(G)} L(\btau). $$ 
\end{problem}

In the problem above, we simply replaced the marginal polytope $\M(\V)$ from our original problem\footnote{If $G$ supports $\C$, we can assume without loss of generality that \cref{prob:marginal} was defined on $\M(\V)$ instead of $\M(\C)$. In particular, the loss function $L$ can be written to depend on marginals $(\btau_{r'})_{r' \in \V}$ instead of $(\btau_r)_{r \in \C}$, because the latter can be computed from the former.} with the local polytope $\L(G)$. Since this is a convex optimization problem with linear constraints, it can be solved with a number of general purpose techniques, including interior point and active set methods \cite{boyd2004convex}.  However, these methods do nothing to exploit the special structure in the constraint set $\L(G)$, and as such, they have trouble running on large-scale problems.  

Our first contribution is to show that we can solve \cref{prob:convex} efficiently by instantiating \prox with a carefully chosen approximate marginal oracle.  To do so, it is useful to view the problem of approximate marginal inference through the lens of the free energy minimization problem, stated below.

\begin{problem}[Approximate Free Energy Minimization] \label{prob:energy}
Let $G$ be a region graph, $\btheta = (\btheta_r)_{r \in V}$ be real-valued parameters, and $H_{\kappa}(\btau) = \sum_{r \in V} \kappa_r H(\btau_r) $, where $\kappa_r \in \mathbb{R}$ are counting numbers, and $H(\btau_r) = -\sum_{\x_r \in \dom_r} \btau_r(\x_r) \log{\btau_r(\x_r)}$ is the Shannon entropy of $\btau_r$.
%
$$ \hat{\btau} = \argmin_{\btau \in \L(G)} -\btau^{\top} \btheta - H_{\kappa}(\btau) $$
\end{problem}

This problem approximates the (intractable) variational free energy minimization problem~\cite{wainwright2008graphical}, for which the optimum gives the true marginals of $\p_\btheta$, by using $\L(G)$ instead of $\M(\V)$, and using $H_{\kappa}(\btau)$ as an approximation to the full Shannon entropy.
%\ds{TODO: add sentence here to connect to exact inference} If $G$ is a Junction Tree, and the counting numbers $\counting$ are chosen appropriately, then it can be shown that the marginals of the graphical model with parameters $\btheta$ exactly solve \cref{prob:energy}.
Many algorithms for approximate marginal inference can be seen as solving variants of this free energy minimization problem under different assumptions about $G$ and $\counting$ \cite{heskes2004uniqueness,wainwright2003tree,wiegerinck2005approximations,loh2014concavity,hazan2012tightening,yedidia2005constructing,hazan2012convergent,meltzer2012convergent,heskes2006convexity,heskes2003generalized,pakzad2005estimation}.  %\ds{The rest of this paragraph has background that may not be needed. Consider dropping parts about Bethe and loopy BP especially, maybe also TRW. Add citations for statements like ``many algorithms can be seen as...''} Indeed, one of the most famous approximate inference algorithms, \emph{loopy belief propagation} on a factor graph, falls into this category.  In particular, if loopy belief propagation converges, it converges to a fixed point of \cref{prob:energy}, where $\counting$ correspond to the Bethe-entropy approximation.  Unfortunately, the Bethe entropy is not convex except in special cases, and loopy belief propagation is not guaranteed to converge in general.  For this reason, variants of loopy belief propagation have been proposed that can be shown to solve \cref{prob:energy} where $\counting$ are \emph{convex} counting numbers (i.e., they correspond to a convex entropy approximation).  One well-known algorithm from this class is tree-reweighted belief propagation \cite{wainwright2003tree}.  However, this algorithm is only applicable for pairwise models (i.e., $|r| \leq 2$ for all $ r \in V$).  A more general but lesser-known algorithm was proposed by Hazan et al. \cite{hazan2012tightening} and is shown in \cref{alg:mpconvex}.  Other related algorithms for this problem also exist \cite{wiegerinck2005approximations,loh2014concavity}. 

\begin{theorem}[Algorithm for Approximate Free Energy Minimization \cite{hazan2012tightening}] \label{thm:energy}
Given a region graph $G$, parameters $\btheta = (\btheta_r)_{r \in \V}$, and any positive counting numbers $\counting_r > 0$ for $ r \in \V$, \gbp solves the approximate free energy minimization problem of \cref{prob:energy}.  
\end{theorem}

Importantly, the complexity of \cref{alg:mpconvex} depends mainly on the size of the largest clique in the region graph.  In many cases of practical interest, this will be exponentially smaller in the saturated region graph than in a junction tree. %\ds{Suggest jumping straight from here to Theorem.} %One limitation of \cref{alg:mpconvex} is that its correctness depends on every counting number being positive.  This is somewhat unnatural, because when $G$ is a junction tree, exact marginal inference solves \cref{prob:energy} with positive and negative counting numbers.  Hence, \cref{alg:mpconvex} does not reduce to ordinary belief propagation when $G$ is a junction tree.  Remarkably, this drawback will not matter for our purposes, as we show in \cref{thm:approx}  

\begin{theorem} \label{thm:approx}
When \prox uses \gbp as the \oracle (with \textbf{any} positive counting numbers $\kappa$), it solves the convex optimization problem over the local polytope of \cref{prob:convex}.
\end{theorem}

This result is remarkable in light of previous work, where different counting number schemes are used with the goal of tightly approximating the true entropy, and form the basis for different approximate inference methods. In our setting, all methods with \emph{convex} counting numbers are equivalent: they may lead to different \emph{parameters} $\hat\btheta$, but the corresponding pseudo-marginals $\hat\btau = \gbp(\hat\btheta)$ are invariant. Indeed, the optimal $\hat\btau$ depends only on the estimation objective $L(\btau)$ and the structure of the local polytope. We conjecture that a similar invariance holds for traditional marginal-based learning objectives with approximate inference~\cite{domke2013learning} when message-passing algorithms based on convex free-energy approximations are used as the approximate inference method.

\begin{proof}
Since $L$ is a convex function and $\L$ is a convex constraint set, this problem can be solved with mirror descent \cite{beck2003mirror}.  Each iteration of mirror descent requires solving subproblems of the form:
%
$$\btau^{t+1} = \argmin_{\btau \in \L} \btau^{\top} \grad L(\btau^t) + \frac{1}{\eta_t} D(\btau, \btau^t) \quad\quad D(\btau, \btau^t) = \psi(\btau) - \psi(\btau^t) - (\btau - \btau^t)^{\top} \grad \psi(\btau^t)$$
%
Here, $D$ is a Bregman distance measure and $\psi$ is some strongly convex and continuously differentiable function.  Setting $ \psi = -H_{\counting}$, a negative weighted entropy with any (strongly) convex counting numbers $\counting$, we arrive at the following update equation:
%
\begin{align*}
%\btau^{t+1} &= \argmin_{\btau \in \L} \btau^{\top} \grad L(\btau^t) + \frac{1}{\eta_t} D(\btau, \btau^t) \\
\btau^{t+1} &= \argmin_{\btau \in \L(G)} \btau^{\top} \grad L(\btau^t) + \frac{1}{\eta_t} \Big( -H(\btau) + H(\btau^t) + (\btau - \btau^t)^{\top} \grad H_{\counting}(\btau^t) \Big) \\
%&= \argmin_{\btau \in \L} \btau^{\top} \grad L(\btau^t) + \frac{1}{\eta_t} \Big( -H_{\rho}(\btau) + \btau^T \grad H_{\rho}(\btau^t) \Big) \\
%&= \argmin_{\btau \in \L} \btau^{\top} \Big(\grad L(\btau^t) + \frac{1}{\eta_t} \grad H_{\rho}(\btau^t) \Big) - \frac{1}{\eta_t} H_{\rho}(\btau) \\
&= \argmin_{\btau \in \L(G)} \btau^{\top} \Big(\eta_t \grad L(\btau^t) + \grad H_{\counting}(\btau^t) \Big) - H_{\counting}(\btau) \tag{algebraic manipulation} \\
&= \argmin_{\btau \in \L(G)} \btau^{\top} \Big(\eta_t \grad L(\btau^t) - \btheta^t \Big) - H_{\counting}(\btau) \tag{\ds{TODO}} \\
%&= \btau \big( -\eta_t \grad L(\btau^t) - \grad H(\btau^t) \big) \\
&= \gbp \big(G, \btheta^t -\eta_t \grad L(\btau^t), \counting \big) \tag{\cref{thm:energy}}
\end{align*}
%
\end{proof}

\begin{algorithm}
%\caption{Message Passing for Convex Free Energy on a Region Graph \cite{hazan2012tightening}} \label{alg:mpconvex}
\caption{\gbp \cite{hazan2012tightening}} \label{alg:mpconvex}
\begin{algorithmic}
\STATE {\bfseries Input:} Region Graph $G=(V,E)$, parameters $\btheta = (\btheta_r)_{r \in V}$, convex counting numbers $\counting_r > 0$
\STATE {\bfseries Output:} Model marginals $\btau = (\btau_r)_{r \in \C}$
\STATE $\counting_{r,t} = \counting_r / (\counting_t + \sum_{p \rightarrow t} \counting_p)$
\STATE Initialize $m_{r\rightarrow t}(\x_t) = 0$ and $\lambda_{t \rightarrow r}(\x_t) = 0$
\FOR{$i = 1,\dots$}
\FOR{$r \rightarrow t$}
\STATE $m_{r \rightarrow t}(\x_t) = \counting_r \log{\Big( \sum_{\x_r \setminus \x_t} \exp{\Big( (\btheta_r(\x_r) + \sum_{c \neq r} \lambda_{c \rightarrow r}(\x_c) - \sum_{p} \lambda_{r \rightarrow p}}(\x_p))/\counting_r)\Big)\Big)}$
\STATE $\lambda_{t \rightarrow r}(\x_t) = \counting_{r,t} \Big( \btheta_t(\x_t) + \sum_{c} \lambda_{c \rightarrow t}(\x_t) + \sum_{p} m_{p \rightarrow t}(\x_t) \Big) - m_{t \rightarrow r}(\x_t)$
\ENDFOR
\ENDFOR
\FOR{$r \in \C$}
\STATE $\btau_r(\x_r) \propto \exp{\Big((\btheta_r(\x_r) + \sum_{t} \lambda_{t \rightarrow r}(\x_t) - \sum_p \lambda_{r \rightarrow p}(\x_r))/\counting_r\Big)}$
\ENDFOR
\RETURN $\btau = (\btau_r)_{r \in V}$
\end{algorithmic}
\end{algorithm}


\subsection{Inference: Answering New Queries}

We now turn our attention to the problem of inference.  The central challenge is to estimate out-of-clique marginals.  That is, we want to estimate $\btau_r$ where $r \not \in \C$.  Previously, we accomplished this by computing the marginal of $\p_{\btheta}$. Unfortunately, that approach no longer makes sense here, because (1) variable elimination in $\p_{\btheta}$ is intractable for the class of models we are interested in, and (2) even if it was tractable, it would give the ``wrong'' answer, since the true marginals of the graphical model with parameter $\btheta$ will be different from the ones estimated in \prox (in this case, the true marginals are not the correct ones), and the difference may be substantial for some choices of convex counting numbers $\counting$.

We thus propose two different methods that do not have these drawbacks, and discuss their benefits and drawbacks.  We expand on this discussion, and consider even more alternatives in the supplement.   

\textbf{Running \prox over an expanded region graph.}  Recall that \prox solves \cref{prob:convex} for \emph{any} region graph that supports $\C$ \footnote{note that the problem itself is slightly different for different region graphs, because the definition of the local polytope depends on the choice of region graph.}.  By default, we use the saturated region graph of $\C$, which is in some sense the smallest graph that encodes all internal consistency constraints.  However, we can expand this region graph to include new vertices and edges corresponding to the cliques whose marginals we want to estimate, even if the loss function does not depend on those marginals.  Clearly, the new region graph is still valid, and \gbp over this graph will return all desired marginals.

The additional cliques do not affect the loss function (the gradient and log-potentials will always remain $\mathbf{0}$ for the new cliques), but they do impact the constraints.  Upon convergence, the estimated pseudo-marginals will belong to the local polytope of the expanded region graph, and hence they will all be locally consistent.  

However, this approach comes at a potentially high cost, since the region graph contains more vertices and edges, each iteration of \prox requires more time, and the algorithm as a whole is slower than it otherwise would be.   This can be especially potent if we wanted to estimate all 3-way marginals, and only measured 10 of them.  This approach adds a significant number of vertices and edges to the region graph, and substantially slows down \gbp and consequently \prox as well.

\textbf{Minimizing Constraint Violation and Maximizing Entropy}
In light of the drawback of the previous approach, we propose a new method which does not require running \prox over a larger region graph.  This approach is a simple post-processing of the output of \prox run over the original region graph, and it can be easily parallelized as well.  For a given clique $r \not \in \V_+$, we would like choose $\btau_r$ to (1) be internally consistent with the existing pseudo-marginals $\btau$ and (2) to maximize entropy among all internally consistent choices.  However, it is certainly possible that there are \emph{no} choices of $\btau_r$ that are internally consistent with $\btau$ (see Example 4.1 in \cite{wainwright2008graphical}).  Thus, we propose the following instead: (1) choose $\btau_r$ to minimize some natural quantification of the constraint violation, and (2) among choices that minimize this quantity, select the one with maximum entropy.  We begin by formalizing the first problem, and then discuss our solution to it, which solves the second problem ``for free''.

\begin{problem}[Minimizing Constraint Violation] \label{prob:project}
Let $\btau = (\btau_r)_{r \in \V}$ and let $ r \not \in \V_+$.
$$ \btau'_r = \argmin_{\btau_r \in \S} \sum_{t,s \in \mathcal{B}} \norm{P_{r \rightarrow s} \btau_r - P_{t \rightarrow s} \btau_s}_2^2 $$
where $\S = \set{ \btau_r \geq 0 \mid \mathbf{1}^{\top} \btau_r = 1}$ is the probability simplex, and $\mathcal{B} = \set{(t, t \cap r) \mid t \in \V}$.
\end{problem}




This is a quadratic minimization problem over the probability simplex.  It can be readily solved with iterative proximal algorithms like entropic mirror descent \cite{beck2003mirror}.   Entropic mirror descent guarantees the solution found will have maximum entropy among all minimizers of the objective.  Additionally, this method does not require any information about attributes not in $r$, and even though it is an iterative algorithm, each iteration runs much faster than an iteration of $\gbp$.  Additionally, if we want to estimate many new marginals, each one can be done in parallel, as the optimization problems do not depend on each other.


==> approach_old.tex <==
\section{Approach}

\setlength{\textfloatsep}{15pt}
\begin{algorithm}[tb]
    \caption{Proximal Estimation Algorithm} \label{alg:proximal}
\begin{algorithmic}
    \STATE {\bfseries Input:} Convex loss function $L(\bmu)$
    \STATE {\bfseries Output:} Estimated marginals $\hat{\bmu}$ %Estimated data distribution $\hat{\p}_{\btheta}$
    \STATE $\btheta = \vect{0}$
    \FOR{$t=1, \dots, T$}
        \STATE $\bmu = \oracle(\btheta)$
        \STATE $\btheta = \btheta - \eta_t \grad L(\bmu)$
    \ENDFOR
    \STATE {\bfseries return} $\bmu$%, $\hat{\p}_{\btheta}$
\end{algorithmic}
\end{algorithm}


In previous work, the key subroutine that needed to be solved is 

$$ \hat{\bmu} = \argmin_{\bmu \in \marg} L(\bmu) $$

One algorithm for solving this problem is stated in \cref{alg:proximal}.  It requires repeated calls to a so-called ``marginal oracle'', which is a routine for computing the marginals of a graphical model $\p_{\btheta}$.  Thus, the efficiency of this algorithm ultimately depends on the efficiency of the marginal oracle.  The complexity of exact marginal inference depends on the structure of the graphical model, so this method breaks down for dense graphical models.  

A natural idea to overcome this scalability limitation is to replace the exact marginal oracle with an approximate one that can run even for dense graphical models.  This is a very appealing idea, but does it make sense?  Remarkably, \cref{thm:approx} shows that if the marginal oracle is chosen carefully, \cref{alg:proximal} solves a very natural relaxation of the original problem.  

\begin{theorem} \label{thm:approx}
When run using \cref{alg:mpconvex} as the marginal oracle, \cref{alg:proximal} solves the following optimization problem:
$$ \hat{\bmu} = \argmin_{\bmu \in \L} L(\bmu) $$
Here, $\L$ is the local polytope defined in \cref{eq:local}.
\end{theorem}

\begin{proof}
First note that $L$ is a convex function of $\bmu$ and $\L$ is a convex set of constraints.  Therefore, this problem can be solved with mirror descent \cite{beck2003mirror}.  Each iteration of mirror descent requires solving subproblems of the form:
%
$$\bmu^{t+1} = \argmin_{\bmu \in \L} \bmu^{\top} \grad L(\bmu^t) + \frac{1}{\eta_t} D(\bmu, \bmu^t)$$
%
Where $D$ is a Bregman distance measure defined as
%
$$D(\bmu, \bmu^t) = \psi(\bmu) - \psi(\bmu^t) - (\bmu - \bmu^t)^{\top} \grad \psi(\bmu^t)$$
%
for some strongly convex and continuously differentiable function $\psi$.  Using $ \psi = -H_{\rho}$ to be the negative weighted Kikuchi entropy defined in \cref{eq:kikuchi} with any (strongly) convex counting numbers $\rho$, we arrive at the following update equation:
%
\begin{align*}
\bmu^{t+1} &= \argmin_{\bmu \in \L} \bmu^{\top} \grad L(\bmu^t) + \frac{1}{\eta_t} D(\bmu, \bmu^t) \\
%\bmu^{t+1} &= \argmin_{\bmu \in \marg} \bmu^T \grad L(\bmu^t) + \frac{1}{\eta_t} \Big( -H(\bmu) + H(\bmu^t) + (\bmu - \bmu^t)^T \grad H(\bmu^t) \Big) \\
&= \argmin_{\bmu \in \L} \bmu^{\top} \grad L(\bmu^t) + \frac{1}{\eta_t} \Big( -H_{\rho}(\bmu) + \bmu^T \grad H_{\rho}(\bmu^t) \Big) \\
&= \argmin_{\bmu \in \L} \bmu^{\top} \Big(\grad L(\bmu^t) + \frac{1}{\eta_t} \grad H_{\rho}(\bmu^t) \Big) - \frac{1}{\eta_t} H_{\rho}(\bmu) \\
&= \argmin_{\bmu \in \L} \bmu^{\top} \Big(\eta_t \grad L(\bmu^t) + \grad H_{\rho}(\bmu^t) \Big) - H_{\rho}(\bmu) \\
&= \argmin_{\bmu \in \L} \bmu^{\top} \Big(\eta_t \grad L(\bmu^t) - \btheta^t \Big) - H_{\rho}(\bmu) \\
%&= \bmu \big( -\eta_t \grad L(\bmu^t) - \grad H(\bmu^t) \big) \\
&= \text{\cref{alg:mpconvex}} \big( \btheta^t -\eta_t \grad L(\bmu^t), \rho \big)
\end{align*}
%
The first four steps are simple algebraic manipulation of the original update equation.  The fifth step uses the observation that $ \grad H(\bmu^t) = -\btheta^t $.  This follows from convex duality \ds{say something here}.
Step six follows from the fact that \cref{alg:mpconvex}($\btheta, \rho$) solves the free energy minimization problem $\bmu = \argmin_{\bmu \in \L} -\bmu^T \btheta - H_{\rho}(\bmu)$.
\end{proof}

\subsection{Estimating New Queries}

Once we obtain an estimate $\hat{\bmu}$, we may be interested in estimating new marginals that weren't in the original model, i.e., we want to estimate $\bmu_r$ where $r \not\in \C$.  Previously, this could be done by using the graphical model parameters $\btheta$ obtained in \cref{alg:proximal}, and running variable elimination in the graphical model.  However, there are two problems with applying that idea here.  First, variable elimination will not in general be tractable for the graphical models we may encounter.  Second, even though \cref{alg:proximal} finds the optimal $\bmu$ no matter what convex counting numbers are used in the entropy approximation, different choices of counting numbers will lead to different parameter vectors $\btheta$.   Moreover, the true marginals of the graphical model with parameter $\btheta$ will be different from the ones estimated in \cref{alg:proximal}, and the difference may be substantial for some choices of convex counting numbers $\kappa$. 


Ideally, we'd like to use a maximum entropy criteria to estimate $\bmu_r$.  In particular, $\bmu_r$ should have maximum entropy among all choices that are consistent with every marginal in $\hat{\bmu}$.  However, because the estimated marginals only satisfy the local consistency constraints implied by the region graph, such a marginal may not exist.  See \cite{wainwright2008graphical} for an example.  Due to the possibility of non-existence, one option is to simply settle for some inconsistency on the new marginal. 


==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Checklist
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes
  \item Did you describe the limitations of your work?
    \answerYes{See \cref{sec:limitations}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes
	\item Did you include complete proofs of all theoretical results?
    \answerYes \dsedit{Proofs omitted from the main text are in the supplemental material.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes \dsedit{The code appears in the supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes \dsedit{See Section~\ref{sec:experiments} and Appendix \ref{sec:extraexp}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Repeated 5 trials in every plot, most of the time the variation was too small to be perceptible, although you can see slight variation if you zoom in closely}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{For scalability plots, provided relevant details about computational time and hardware used.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes
  \item Did you mention the license of the assets?
    \answerNo{Licenses of \dsedit{open-source code assets we used are} available in repositories of the cited work. \dsedit{We will release our code with a suitable open-source license upon publication.}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo %{See supplemental material. \ds{Should this be NO? Do you mean the code? I would say for now we are not releasing this as an asset.}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA
\end{enumerate}

\end{enumerate}


==> dan-technical.tex <==
\section{Notation and setup}\label{notation-and-setup}

\subsection{General}\label{general}

\begin{itemize}
\item
  \(\I\{ \cdot \}\) is indicator function.
\item
  \([m] = \{1, 2, \ldots, m\}\) for any integer \(m\)
\end{itemize}

\subsection{Individual data records}\label{individual-data-records}

Single record \(\x = (x_1, \ldots, x_d)\)
\begin{itemize}
\item \(x_i\) is \(i\)th attribute
\item \(x_i\) belongs to domain \(\dom_i\), which is finite with \(n_i\) possible values
\item Overall domain is \(\dom = \prod_{i=1}^d \dom_i\), which has size \(n = \prod_{i=1}^d n_i\). This is exponential in the number of attributes \(d\).
\end{itemize}
  
\subsection{Data set and full contingency
table}\label{data-set-and-full-contingency-table}

\(m\) individuals with records \(\x^{(1)}, \ldots, \x^{(m)}\)

Data set \(\mathbf{X} = (\x^{(1)}, \ldots, \x^{(m)})\)

Contingency table \(\p\) counts the number of individuals with record
equal to \(\x\) for each \(\x\) in the domain. Definition:
\[\p(\x) = \sum_{i=1}^m \I\{\x^{(i)}  = \x\}, \quad \forall \x \in \dom\]

(Convention: use \(\p\) to represent contingency tables because
contingency tables and their marginals behave much like probability
tables and their marginals. The main difference is: contingency tables
are non-negative integers and sum to \(m\); probabilities are
non-negative real numbers and sum to \(1\).)

We will consider \(\p\) to be a vector in \(\R^{n}\) with index set
\(\dom\) (say, ordered lexicographically)

\subsection{Marginals}\label{marginals}

Let \(A \subseteq [d]\) be a generic subset of attributes. Define:

\begin{itemize}
\item
  \(\x_A = (x_i)_{i \in A}\) to be the subvector of \(\x\) restricted to
  attributes in \(A\)
\item
  \(\dom_A = \prod_{i \in A} \dom_i\) be the restricted domain, with
  size \(n_A = \prod_{i \in A} n_i\)
\item
  Let \(-A = [m]\setminus A\) be the complement of \(A\)
\end{itemize}

Define the marignal contingency table (or just ``marginal'') \(\bmu_A\)
as \[
  \bmu_A(\x_A) = \sum_{i=1}^m \I\{ \x^{(i)}_A = \x_A\}
  \]

Note that \(\bmu_A(\x_A)\) is a linear function of \(\p\): \[
  \bmu_A(\x_A) = \sum_{\x_{-A}\in \dom_{-A}} \p(\x_{A}, \x_{-A})
  \] so there exists a matrix \(M_A \in \R^{n_A \times n}\) such that
\(\bmu_A = M_A\p\).

\textbf{(Q: Do you want to use bold or mathbb for matrices?)}

\subsection{Queries}\label{queries}

A linear query is a vector \(\q\) with answer \(\q^T \p\).

A set of \(r\) linear queries \(\q_1, \ldots, \q_r\) can be arranged in
a matrix \(Q \in \R^{r \times n}\) with \(i\)th row equal to \(\q_i\).

The vector of answers to the queries is \(Q \p\).

\(Q\) is the set of \emph{measurement queries}

\subsection{Queries over marginals}\label{queries-over-marginals}

A query may depend only on the marginal table \(\bmu_A\) for a subset
\(A\) of attributes. In this case we write the query as
\(\q_A \in \R^{n_A}\) and the answer is \(\q_A^T \bmu_A\).

(If needed: write \(\q_{A,i}\) if we need to index multiple queries.)

(Optional: A query \(\q\) can be written this way if it can be expressed
as \(\q = M_A^T \q_A\). Then \[
  \q^T \p = \q_A^T M_A \p = \q_A^T \bmu_A
  \] This means \(\q\) is in the row space of \(M_A\). Additional
interpretation?)

\subsection{Measurement cliques}\label{measurement-cliques}

Assume each measurement query depends only on the marginal \(\bmu_C\)
for some \(C \in \C\), where \(\C\) is a collection of cliques (subsets
of attributes). We refer to the collection \(\C\) as the
\emph{measurement cliques}.

There are \(r_C\) total queries for clique \(C\), given in the rows of
the matrix \(Q_C \in \R^{r_C \times n_C}\).

We observe answers \(\y_C = Q_C \bmu_C + \text{Lap}(\Delta_C/\epsilon)\)
for each \(C\). (Check this. Describe sensitivity \(\Delta_C\).)

Let \(\y = (\y_C)_{C \in \C}\) be the complete set of answers to
measurement queries (the concatenation of the query answers from each
clique). Let \(\bmu = (\bmu_C)_{C \in \C}\) be the complete set of
marginals for those cliques.

(Optional: there is a matrix \(M\) such that \(\bmu = M \p\). It is
obtained by stacking the matrices \(M_C\) for all \(C \in \C\).)

\textbf{Observation}: measurements \(\y\) depend only on \(\bmu\), which
is much lower dimensional than \(\p\).

\textbf{Terminology summary} (refine if needed):

\begin{itemize}
\item Measurement cliques \(\C\)
\item Measurement marginals \(\bmu = (\bmu_C)_{C \in \C}\)
\item Measurement queries \(Q = \{Q_C\}_{C \in \C}\)
\item Measurements \(\y = (\y_C)_{C \in \C}\)
\end{itemize}

%\section{Approach}\label{approach}
%
%\subsection{Optimization for
%Estimation}\label{optimization-for-estimation}
%
%We observe \(\y\) (as defined above) and want to answer a target query
%\(\q\). (For now assume we are answering just one arbitrary test query.
%Later we will discuss answering many queries or queries with more
%structure.) We either didn't ask \(\q\) directly, or we did ask it but
%want to use \emph{all} of the available information to estimate
%\(\q^T \p\) as opposed to just using the noisy answer we got.
%
%What principle can we follow? The goal of ``inference'' in DP is to
%estimate \(\hat{\p} \approx \p\) using all available information and
%then use \(\hat{\p}\) to answer later queries. (Cite previous papers.)
%We will refine the terminology to call finding \(\hat{\p}\)
%\emph{estimation}, and using \(\hat{\p}\) to answer the target query
%\emph{inference}. (This matches graphical model terminology.)
%
%The standard framework for estimation and inference uses optimization to
%find \(\hat{\p}\): \[
%\hat{\p}= \argmin_{\p \in \mathcal{S}} F(\p; \y), \qquad \text{answer} = \q^T \hat{\p}
%\]
%
%\begin{itemize}
%\item
%  \(\mathcal{S} = \big\{ \p: \p \geq 0, \mathbf{1}^T \p = m\big\}\) is
%  the (scaled) probability simplex. We relaxed counts from integers to
%  real numbers.
%\item
%  \(F(\p; \y)\) is a loss function. We will usually just write
%  \(F(\p)\).
%\item
%  Examples include L2 and L1
%\item
%  L1 corresponds to a maximum-likelihood criterion
%\item
%  Point out that ``L1'' can use different weights to model MLE when the
%  different queries had different amounts of noise added
%\end{itemize}
%
%\textbf{Problem}: this doesn't scale to high dimensions. The size of
%\(\p\) is exponential in \(d\), and we have to construct it as an
%intermediate step even if the inputs and outputs are small, e.g., if all
%measurement queries and the target query are low-dimensional. (This
%really happens.)
%
%\subsection{Optimization in Terms of
%Marginals}\label{optimization-in-terms-of-marginals}
%
%Assume the loss only depends on measurement marginals \(\bmu\):
%\[
%F(\p; \y) = L(\bmu(\p); \y)
%\]
%
%\begin{itemize}
%\item
%  Again, we will usually just write \(L(\bmu)\)
%\item
%  Examples: L1 or L2 with the measurement queries we described. Give details.
%\item
%  The loss will often have the structure
%  \[ L(\bmu) = \sum_{C \in \C} L_C(\bmu_C)\]
%  but it is not required for our methods.
%\end{itemize}
%
%An ``obvious'' idea would be just to estimate the measurement marginals:
%\[
%\hat{\bmu}= \argmin_{\bmu \in \M} L(\bmu), \qquad \text{answer} = ???
%\]
%
%\begin{itemize}
%\item
%  \(\M = \big\{ \bmu: \exists \p \in \mathcal{S} \text{ with marginals } \bmu \big\}\)
%  is the marginal polytope
%\end{itemize}
%
%The problem with this is that it doesn't tell us how to answer a new
%query, unless that query happens to depend only on some measurement
%marginal \(\bmu_C\).
%
%% I no longer think the next statements are relevant / appropriate.
%%Second, even for queries that are determined by a measurement marginal \(\bmu_C\), it is unclear what criterion is being used to answer the query.
%% For example, the constraint set implies that \emph{some} information from other cliques is being used to estimate \(\bmu_C\), but how, exactly, is this information ``transferred'' to the estimate \(\hat{\bmu}_C\)?
%
%\subsection{\texorpdfstring{Factored \(\p\) and Maximum Entropy
%Criterion}{Factored \textbackslash{}p and Maximum Entropy Criterion}}\label{factored-p-and-maximum-entropy-criterion}
%
%Our solution: we will show that, given a solution
%\(\hat{\bmu} \in \argmin_{\bmu \in \M} L(\bmu)\), we can find a
%distribution \(\hat{\p}\) that has maximum entropy among all
%distributions with marginals \(\hat{\bmu}\). Because it is factored, we
%can represent \(\hat{\p}\) compactly and use it to answer new queries
%efficeintly.
%
%\textbf{Factored distributions (graphical models)}. Let
%\(\p(\x; \btheta) = \frac{1}{Z} \sum_{C \in \C} \exp( \btheta_C(\x_C) )\).
%This distribution is a graphical model that factors over the clique set
%\(\C\). The vector \(\btheta = (\btheta_C)_{C \in \C}\) comprises the
%parameters of the graphical model.
%
%\textbf{Theorem} (imprecise). Let
%\(\hat{\bmu} \in \argmin_{\bmu \in \M} L(\bmu)\). We can compute
%parameters \(\hat{\btheta}(\hat{\bmu})\) such that
%\(p(\x; \hat{\btheta}(\hat{\bmu}))\) has maximum entropy among all
%distributions with marginals \(\hat{\bmu}\). The parameters are not
%uniquely determined by \(\hat{\bmu}\) but the distribution
%\(\p(\x; \hat{\btheta}(\hat{\bmu}))\) is uniquely determined.
%
%\textbf{Technical notes}
%
%\begin{itemize}
%\item
%  As stated this is basically a direct consequence of standard marginal
%  polytope stuff from Wainwright and Jordan (Theorem 3.4 and surrounding
%  content)
%\item
%  There is a technicality: the theorem as stated only applies if
%  \(\hat{\bmu}\) is in the \emph{interior} of the marginal polytope.
%  Specifically this means it has no zeros. We need to figure out what to
%  say if \(\hat{\bmu}\) has zeros. I hope there will be a satisfactory
%  precise statement. Something like: there is a sequence of
%  values\ldots{} (see part (a) of Theorem 3.4).
%\item
%  \textbf{Ideally we'd like a stronger statement}: we can find a
%  factored distribution that has maximum entropy among all distributions
%  with marginals that minimize \(L(\bmu)\). Mathematically it would look
%  something like this: \[
%    \p(\x; \hat{\btheta}) \in \argmax_{\p \in \mathcal{S}} H(\p) \quad \text{s.t. } \, \bmu(\p) \in \argmin_{\bmu \in \M} L(\bmu)
%    \] The reason we don't obviously get this is because if \(L(\bmu)\)
%  has multiple minima, we might choose one minimum \(\hat{\bmu}\) that
%  leads to lower entropy than if we had chosen a different one. If
%  \(L(\bmu)\) is strictly convex, it has a single minimum and we get
%  what we want. There's a chance that we get the stronger property
%  defined by the way we solve the problem (e.g., the proximal method)
%  but this is something we'd have to analyze much more carefully.
%\item
%  TODO: Dan come back and resolve as much of this as possible. Ryan,
%  feel free to take a crack at it if you want.
%\end{itemize}
%
%\section{Algorithms}\label{algorithms}
%
%\subsection{Estimation}\label{estimation}
%
%We need algorithms to find \(\hat{\bmu}\) and \(\hat{\btheta}\). We have
%two approaches, the ``direct method'' (need a better name for this) and
%a proximal method.
%
%\subsubsection{Direct Method}\label{direct-method}
%
%Describe direct method where we parameterize the marginals
%\(\bmu(\btheta)\) as a function of \(\btheta\) and then solve: \[
%\min_{\btheta} L\big( \bmu(\btheta) \big)
%\]
%
%\begin{itemize}
%\item
%  Pro: no constraints
%\item
%  Pro: can compute derivatives etc. using message passing
%\item
%  Con: not convex!
%\end{itemize}
%
%Give as many details as necessary. Cite Domke. Can defer stuff to
%appendix.
%
%\subsubsection{Proximal Method}\label{proximal-method}
%
%Describe proximal method. Directly solve
%\(\argmin_{\bmu \in \M} L(\bmu)\) using a variant of entropic mirror
%descent (or regularized dual averaging?). Cite Vilnis et al.
%
%\begin{itemize}
%\item
%  Pro: convex, guaranteed convergence
%\item
%  Pro: recover \(\hat{\btheta}\) ``for free''
%\item
%  Con: sometimes slower?
%\end{itemize}
%
%\subsection{Inference}\label{inference}
%
%Describe the class of target queries we can support. Give basic
%notation, etc.
%
%Describe the novel variant of variable elimination to compute these
%queries.
%
%\section{Extras}\label{extras}
%
%\subsection{Nonlinear queries}\label{nonlinear-queries}
%
%The method applies to nonlinear queries over marginals. Write a single
%such query as \(\q_A(\bmu_A)\) where \(\q_A: \R^{n_A} \to \R\). Our
%algorithm needs only \(\grad {\q_A}\).
%
%(optional) Write a batch of nonlinear queries as \(Q_A(\bmu_A)\) where
%\(Q_A: \R^{n_A} \to \R^{r_A}\). Our algorithm needs the Jacobian of
%\(Q_A\).
%
%This means \(\q_A\) and \(Q_A\) need to be continuous and
%differentiable.


==> experiments_old.tex <==
\section{Experiments} \label{sec:experiments}

\ry{this section will need to be restructured quite a bit}
\ry{can we combine related work and experiments? As we will compare against related work}
\ry{also, plots are hard to read in black and white}

Next we evaluate empirically the efficiency and accuracy of our proposed methods.  All experiments are performed on a quad-core Intel i7 3.6 GHz processor with 16 GB of RAM.  

For the efficiency experiments, we used synthetic data, allowing us to systematically vary the domain size and number of dimensions of the data and evaluate their impact.  Specifically, we consider a dataset with 1 million tuples and $d$ variables, each with domain size $n_i = 10$. We vary $d = 2 \dots 16 $. We consider chain structured measurements, which include the $\{ i, i+1 \}$ marginals for $ 1 \leq i \leq d-1 $.  

For accuracy experiments, we use the Adult dataset obtained from the UCI machine learning repository \cite{Dua:2017}, which contains 32,561 tuples and 11 discrete (or appropriately discretized) attributes: age, workclass, education, marital status, occupation, relationship to householder, race, sex, hours-per-week, country, and income>=50K.  The total domain size is $ 100 \times 9 \times 16 \times 7 \times 15 \times 6 \times 5 \times 2 \times 100 \times 42 \times 2 \approx 7.6 \times 10^{11} $.  

\begin{figure}[t]
\centering
\subcaptionbox{\label{fig:chain} Model estimation from measurements}{\includegraphics[width=0.45\textwidth]{fig/chain.pdf}}
\subcaptionbox{\label{fig:inference} Target query inference}{\includegraphics[width=0.45\textwidth]{fig/chain_inference.pdf}}
\caption{The runtime of model estimation and inference as dimensionality grows.} \label{fig:efficiency}
\end{figure}


%\ry{I'm wondering if these things can be moved to related work}
% GM: I don't think so, but we could try to shorten if we need to. 

\textbf{Efficiency of estimation.}
Fig. \ref{fig:chain} shows the runtime of our two algorithms for model estimation, Direct and Proximal, compared with two competing methods, LSQR and MW. LSQR \cite{Zhang18Ektelo:} is an iterative algorithm for solving an ordinary least squares problem (without non-negativity constraints); it the most efficient method we are aware of that handles general linear measurements. Least-squares is a very common estimation method in the literature \cite{hay2010boosting,Nikolov13Geometry,li2014data,qardaji2013understanding,ding2011differentially,Xiao10Differential,li2010optimizing}. We use it here to find the minimum-norm $d$-way contingency table which minimizes squared error given the chain-structured measurements.  
%showed that by simply representing the measurements as a sparse matrix and using an iterative conjugate gradient algorithm (such as LSQR) was more efficient in practice.  
MW uses multiplicative weights to repeatedly update an estimate of the full contingency table to reflect the noisy measurements \cite{hardt2012simple}.  While the authors of  \cite{hardt2012simple} describe an enhancement that uses a factored representation, it only applies when the measurements can be partitioned into groups that depend on disjoint subsets of variables.  That enhancement offers no benefit for chain-structured measurements, but would make MW efficient for measurements on disjoint sets of variables.  Nevertheless, our methods do not have such an extreme requirement in order to benefit from the efficiency of a factored representation.

%For measurement sets that can be partitioned in this way, the factored variant of the multiplicative weights algorithm would be more efficient.  Our algorithms would also be efficient in this setting, which shows that our algorithms operate over a factored representation of the data for a more general class of queries than factored multiplicative weights.  

%Although this method can operate on a compact factored representation of $\hat{\p}$ in some cases, for chain-structured measurements it requires materializing the full representation.   

The Direct and Proximal algorithms are both linear in the number of dimensions for chain structured measurements, and as shown in Fig. \ref{fig:chain}, our algorithms are highly scalable, running in a matter of seconds up to $d=16$.  We were unable to run LSQR or MW beyond $d=7$ due to the memory requirements of jointly representing the measurements.  For these methods, the measurements are represented as a sparse matrix, which requires storing $(d-1) \cdot 10^d$ values.  If the measurement queries were represented more compactly, these algorithms may be able to scale up to $d=8$ or $d=9$, but beyond that storing the full contingency table would be impossible on common hardware.


\textbf{Efficiency of inference.}
We now empirically evaluate the inference algorithm we described in Sec.~\ref{inference} to answer factored queries with $\Q_i \in \R^{2 \times n_i}$.  The details of the queries encoded are not important for measuring efficiency, only the size of $\Q_i$ matters.  However, we can interpret this query matrix as compressing the distribution (see supplemental material for more information).    

We compare our inference method (Algorithm~\ref{alg:inference}) to a baseline algorithm that first computes the full contingency table (using the formula from definition~\ref{def:graphical-model}) then answers the queries over the full contingency table.  As shown in Fig. ~\ref{fig:inference}, the baseline breaks down after $ d = 7 $ due to memory limitations, but our algorithm easily scales to $d=16$.   

\textbf{Accuracy of inferred query estimates.}
Next we demonstrate the accuracy improvements afforded by proper inference.  The measurement and target queries, for the Adult dataset, are listed in Fig. ~\ref{table:key}.  There are six carefully chosen low-dimensional query matrices in the measurement set, in addition to the $11$ 1-way marginals (not listed).  The privacy budget of $ \epsilon = 2.0$ is split equally among these $17$ measurement sets.  There are four additional target query matrices.  
The matrix $\P$ in Fig. ~\ref{table:key} contains range queries that characterize the cumulative distribution function, and the matrix $\A$ is a low-sensitivity query matrix from which the answers to range queries can be accurately derived.\cite{li2015matrix} These special query matrices are used for the continuous variables (age and hours-per-week) to demonstrate the important capability of our technology to handle arbitrary measurements of the marginals.
%\ry{for consistency we should consider describing the measurements before the subsections (as we do for chain queries)}

%\gm{below I say 'in-measurement' and 'out-of-measurement' to distinguish the experiments.  Maybe in-clique and out-of-clique are better?}

We evaluate accuracy of our inferred query answers in two settings.  First, we study accuracy on queries that are present in the measurement set (queries 1-6 in Fig.~\ref{table:key}).   Our inferred answers are consistent and incorporate all available evidence.  We compare with a baseline method that simply reports the noisy measurement answer. Second, we study accuracy on queries {\em not} present in the measurement set (queries 7-10 in Fig.~\ref{table:key}).  
%and \gmref{spanning multiple cliques}{I think this point is important: all your measurements are marginals, so there are un-measured queries within cliques, e.g. range queries on a 1-way marginal}.  
Since the first baseline does not apply here, we compare with a different baseline that uses the 1-way marginal measurements and assumes independence among the variables involved in the queries.
%
We used the Proximal algorithm for estimating $\p_{\btheta}$, running it for 2500 iterations (or about 25 seconds) using line search to select the step sizes $t_k$. %Small improvements to accuracy would be possible by running additional iterations. 
We evaluate the quality of a query estimate using the median $L_1$ error over 25 random trials.  The results are shown in Fig. ~\ref{fig:adult1} and ~\ref{fig:adult2}.

\begin{figure}
\centering
\captionsetup{justification=centering}
\subcaptionbox{\label{table:key} Measurement queries (1-6) \\ \hspace{7pt} and target queries (7-10)}{
\resizebox{0.31\textwidth}{!}{%
\begin{tabular}{|c|l|l|}
\hline
\textbf{\#} & \textbf{Clique Variables}                                                      & \textbf{Query Set} \\\hhline{|=|=|=|}
1           & workclass, education                                                           & $\II \otimes \II$              \\
2           & education, income                                                              & $\II \otimes \II$              \\
3           & age, marital status                                                            & $\A \otimes \II$              \\
4           & age, relationship                                                              & $\A \otimes \II$              \\
5           & \begin{tabular}[c]{@{}c@{}}marital status, sex, \\ hours-per-week\end{tabular} & $\II \otimes \II \otimes \A$          \\
6           & race, country                                                                  & $\II \otimes \II$             \\ \hhline{|=|=|=|}
7           & workclass, income                                                              & $\II \otimes \II$              \\
8           & marital status, relationship                                                   & $\II \otimes \II$            \\
9           & relationship, hours-per-week                                                   & $\II \otimes \P$              \\
10          & occupation, sex                                                                & $\II \otimes \II$             \\\hline
\end{tabular}} \vspace{3 mm}
}
\subcaptionbox{\label{fig:adult1} In-measurement \\ \hspace{5pt} target queries}{\includegraphics[width=0.33 \textwidth]{fig/adult1}}
\subcaptionbox{\label{fig:adult2} Out-of-measurement \\ \hspace{-10pt} target queries}{\includegraphics[width=0.33 \textwidth]{fig/adult2}}
\caption{L1 Error from baseline estimates and our estimates.} \label{fig:adult}
\end{figure}

For the in-measurement target queries, we found that our inferred query answers offered lower error than the corresponding baseline on all the measured 2-way and 3-way marginals, usually by a substantial amount.  In result not shown, it also improved the error on 9 out of 11 of the 1-way marginal estimates (the difference in error on the other 2 marginal estimates was negligible).

For the out-of-measurement target queries, our inferred query answers offered meaningful improvements to error for the first three measurements, and a small improvement for the fourth.  This is because the measurement queries contain more information about the first three target queries.  Note that the error of both methods is much worse for out-of-measurement queries because they can not be expressed as a linear combination of the measured queries.  Despite the high error, it is still useful to have better-than-baseline estimates of these quantities.  

Improvements in accuracy stemming from inference have been observed before in the privacy literature (e.g. \cite{hay2010boosting}), however existing inference algorithms are not capable of scaling to the large domain we considered in this experiment.




==> graphical_models.tex <==
\section{Graphical Models}

Graphical models provide an elegant means to encode high-dimensional distributions efficiently, by representing it as a product of low-dimensional factors.  Specifically, a graphical model is a factorized distribution $\p_{\btheta}$, defined by a  collection of cliques $\C$ and an associated parameter vector $\btheta_r$ for each $ r \in \C$.  Here, $\btheta \in \mathbb{R}^{n_r}$ is a vector indexed by domain elements $\x_r \in \Omega_r$.  It assumes the form:

\begin{equation}
\p_{\btheta}(\x) = \frac{1}{Z(\btheta)} \exp \Big(\sum_{r \in \C} \btheta_r(\x_r) \Big)
\end{equation}

Above, $\exp{(\btheta_r)}$ are the factors of the distribution.  

\paragraph*{Marginal Inference}
One of the most important algorithmic problems in graphical models is marginal inference.  That is: how can we efficiently compute a marginal $\bmu_r$ of a graphical model $\p_{\btheta}$?  Naively, one could calculate $\bmu_r$ as follows:

$$ \bmu_r(\x_r) = \sum_{\x \setminus \x_r} p_{\btheta}(\x) $$

where $ \x \setminus \x_r = \set{\x' \in \dom \mid \x'_r = \x_r} $.  This approach is very simple, but since it sums over all elements of the domain, it takes exponential time and is infeasible for high-dimensional domains.  We can often do much better by exploiting the factorization structure of the graphical model.  \emph{Variable elimination} is a general-purpose method that can compute any marginal $\bmu_r$ of a graphical model $\p_{\btheta}$, even if $r \not\in \C$.  It does this efficiently for certain graphical models by rewriting the sum in a particular way that makes the computation tractable.  We are often interested in computing $\bmu_r$ for every $r \in \C$.  While we could simply run variable elimination $| \C |$ times to perform this computation, a better approach is to use \emph{belief propagation} (also called the sum-product algorithm).  Belief propagation computes $\bmu_r$ for all $ r \in \C$ in roughly the same amount of time it takes variable elimination to compute $\bmu_r$ for a single $r \in \C$.   

The complexity of belief propagation depends crucially on the structure of the underlying graphical model.  For tree-structured graphical models, belief propagation runs in linear time with respect to the size of the parameter vector $\btheta$.  However for more complicated models, belief propagation requires first constructing a \emph{Junction Tree} to facilitate exact marginal inference.  This junction tree contains ``super cliques'' which are obtaind by combining densely connected cliques from the original graphical model.  The size of these super cliques ultimately determines the complexity of belief propagation.  In general, their size grows exponentially with the density of the graphical model. Therefore, for belief propagation is not suitable for all graphical models.  For example, the Junction Tree for the the simple graphical model that contains parameters for every pair of attributes $i,j$ would have size equal to the entire domain.  This this does not indicate an inefficiency of belief propagatoin, but of the inherent hardness to marginal inerence in a general graphical model.  Marginal inference is known to be a ???-hard problem.  


\paragraph*{Learning}
Another important problem in graphical models is that of \emph{learning}.  Given a marginal vector $\bmu$, find a graphical model $\p_{\btheta}$ that has those marginals.  Remarkably, such a graphical model always exists, as long as $\bmu$ is strictly positive.  Moreover, this graphical model has maximum entropy among all distributions with marginals $\bmu$.

\begin{theorem}[Maximum entropy] \label{theorem:maxent}
Given any $\hat{\bmu}$ in the interior of $\M$ there is a parameter vector $\hat{\btheta}$ such that the graphical model $\p_{\hat{\btheta}}(\x)$ has maximum entropy among all $\hat{\p}(\x)$
with marginals $\hat{\bmu}$.\footnote{If the marginals are on the boundary of $\M$, e.g., if they contain zeros, there is a sequence of parameters $\{\btheta^{(n)}\}$ such that $\p_{\btheta^{(n)}}(\x)$ converges to the maximum-entropy distribution as $m \to \infty$.}
\end{theorem}

\subsection{Region Graphs and Message Passing Algorithms for Approximate Inference}

Due to the inherent hardness of exact marginal inference, and the importance of the problem, there has been a large body of research around the problem of \emph{approximate marginal inference} in a graphical model.  In this paper we will focus on one small class of approaches to this problem that work by passing messages along edges of a carefully constructed \emph{region graph} that depends on the graphical model.

A region graph is a data structure that facilitates these message passing algorithms.  Region Graphs can encode Junction Trees and Factor graphs as a special case.  A region graph contains a collection of nodes, and each node is labeled with a clique.  Every clique in the graphical model must be contained in some node of the region graph.  
%In general, the set of nodes in the region graph is closed under intersection, i.e., if $r \in \C$ and $s \in \C$ then $r \cap s \in \C$.  
Typically, the cliques of the graphical model will correspond to the maximal cliques in the region graphs, although this is not necessary.  \cref{fig:regions} shows three different region graph structures for a simple graphical model defined over a 5D domain.  \cref{fig:clique} is a junction tree of the graphical model.  It is obtained by merging three overlapping cliques into a single larger clique.  \cref{fig:factor} shows what the Factor graph of this model looks like. It contains one node for every clique in the model, plus nodes for singleton attributes.  A clique node is connected to an attribute node if that attribute is containd within the clique. \cref{fig:region} shows a fully saturated region graph for this model.  It also contains a clique node for every clique in the graphical model, plus smaller cliques which are formed from the intersection of two cliques.  

The structure of the region graph corresponds to the local consistency constraints we wish to enforce between pairs of cliques.  Each edge in the graph can be interpreted as a constraint that marginals agree on shared attributes.   For any region graph, there is an implied \emph{local polytope} which encodes all of these internal consistency constraints expected to hold.  These are contraints are necessary, but not sufficient, for the estimated marginals to be realizable.  In the special case when the region graph is a tree, then the  marginals can be shown to be realizable, and hence in this case the local polytope corresponds to the \emph{marginal polytope}, or the set of all marginals that are realizable from some high-dimensional distribution.    

\begin{equation} \label{eq:localpolytope}
\L =
  \left\{ \bmu \geq 0
  \;\middle\vert\;
  \begin{array}{@{}l@{}l@{}}
  \sum_{\x_r} \bmu_r(\x_r) = 1 & \forall r \in \C \\
  \sum_{\x_r \setminus \x_t} \bmu_r(\x_r) = \bmu_t(\x_t) \quad\quad & \forall r \rightarrow t \in \C\\
  \end{array}
  \right\}
\end{equation}

Unlike the region graphs in \cref{fig:factor,fig:region}, the region graph in \cref{fig:clique} is a tree, and therefore marginals that satisfy the constraints in \cref{eq:localpolytope} are realizable.  However, message passing on the junction tree is not always tractable, and we may be forced to settle for one of the relaxations shown in \cref{fig:factor,fig:region}.  The difference between the factor graph in \cref{fig:factor} and the saturated region graph in \cref{fig:region} is on the constraints involving cliques $\set{A,B,C}$ and $\set{B,C,D}$.  In the factor graph, these two marginals have to agree on the common $B$ marginal and the common $C$ marginal, but not necessarily on the $\set{B,C}$ marginal.  In contrast, the saturated region graph encodes this finer-grained constraint.  The saturated region graph is clearly the more suitable data structure because it captures more of the constraints we know hold on realizable marginals.  On the other hand, message passing algorithms are typically more efficient on factor graphs, so there is a trade-off between efficiency and constraint coverage.  For pairwise graphical models, where every clique has size two \footnote{or more generally, if the overlap between any two pairs of cliques is at most one}, the two graphs are identical.  Pairwise graphical models have recieved considerably more attention than general region  graphs, and there are many approximate marginal inference algorithms that are designed specifically for pairwise models, with no clear extension to general graphs.   In this work, it is important to be able to handle larger clique structures, so we focus out discussion on fully saturated region graphs. 

 

\begin{figure}
  \begin{subfigure}[b]{0.19\textwidth}
    \centering\includegraphics[width=\textwidth]{fig/ex_clique}
    \caption{\label{fig:clique} Junction Tree}
  \end{subfigure}%
  \hspace{2em}
  \begin{subfigure}[b]{0.38\textwidth}
    \centering\includegraphics[width=\textwidth]{fig/ex_factor}
    \caption{\label{fig:factor} Factor Graph}
  \end{subfigure}%
  \hspace{2em}
  \begin{subfigure}[b]{0.38\textwidth}
    \centering\includegraphics[width=\textwidth]{fig/ex_region}
    \caption{\label{fig:region} Saturated Region Graph}
  \end{subfigure}%
\caption{\label{fig:regions} Comparison of different region graph structures for a graphical model defined over a domain with attributes $\set{A,B,C,D,E}$ with cliques $\C = \set{\set{A,B,C}, \set{A,D}, \set{B,C,D}, \set{D,E}}$.}
\end{figure}

\begin{algorithm}
\caption{Belief Propagation on Junction Tree}
\begin{algorithmic}
\STATE {\bfseries Input:} Model parameters $\btheta = (\btheta_r)_{r \in \C}$
\STATE {\bfseries Output:} Model marginals $\bmu = (\bmu_r)_{r \in \C}$
\FOR{$(r,s) \rightarrow t$}
\STATE $m_{r \rightarrow t}(\x_t) = m_{t \rightarrow s}(\x_t) = \log{\Big(\sum_{\x_r \setminus \x_t} \exp{\Big(\btheta_r(\x_r) + \sum_{u \neq t} m_{u \rightarrow r}(\x_u)\Big)} \Big)}$ \\
\ENDFOR
\FOR{$r \in \C$}
\STATE $\bmu_r(\x_r) \propto \exp{\Big(\btheta_r(\x_r) + \sum_{t} m_{t \rightarrow r}(\x_t)\Big)}$
\ENDFOR
\RETURN $\bmu = (\bmu_r)_{r \in \C}$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Message Passing for Convex Free Energy on a Region Graph} \label{alg:mpconvex}
\begin{algorithmic}
\STATE {\bfseries Input:} Model parameters $\btheta = (\btheta_r)_{r \in \C}$, convex counting numbers $c_r > 0$
\STATE {\bfseries Output:} Model marginals $\bmu = (\bmu_r)_{r \in \C}$
\STATE $c_{r,t} = c_r / (c_t + \sum_{p \rightarrow t} c_p)$
\STATE Initialize $m_{r\rightarrow t}(\x_t) = 0$ and $\lambda_{t \rightarrow r}(\x_t) = 0$
\FOR{$i = 1,\dots$}
\FOR{$r \rightarrow t$}
\STATE $m_{r \rightarrow t}(\x_t) = c_r \log{\Big( \sum_{\x_r \setminus \x_t} \exp{\Big( (\btheta_r(\x_r) + \sum_{c \neq r} \lambda_{c \rightarrow r}(\x_c) - \sum_{p} \lambda_{r \rightarrow p}}(\x_p))/c_r)\Big)\Big)}$
\STATE $\lambda_{t \rightarrow r}(\x_t) = c_{r,t} \Big( \btheta_t(\x_t) + \sum_{c} \lambda_{c \rightarrow t}(\x_t) + \sum_{p} m_{p \rightarrow t}(\x_t) \Big) - m_{t \rightarrow r}(\x_t)$
\ENDFOR
\ENDFOR
\FOR{$r \in \C$}
\STATE $\bmu_r(\x_r) \propto \exp{\Big((\btheta_r(\x_r) + \sum_{t} \lambda_{t \rightarrow r}(\x_t) - \sum_p \lambda_{r \rightarrow p}(\x_r))/c_r\Big)}$
\ENDFOR
\RETURN $\bmu = (\bmu_r)_{r \in \C}$
\end{algorithmic}
\end{algorithm}

\subsection{Marginal Inference as Optimization}

Interestingly, marginal inference can be cast as an optimization problem, and algorithms for exact inference like belief propagation solve this optimization problem.  Let $\bmu$ denote the \emph{concatenatd vector of marginals}.    

In particular, it can be shown that the marginals $\bmu(\btheta)$ of the graphical model $\p_{\btheta}$ solve the following constrained optimization problem. 

\begin{equation} \label{eq:energy}
\bmu(\btheta) = \argmin_{\bmu \in \M} -\bmu^T \btheta - H(\bmu)
\end{equation}

The objective function is known as the ``free energy''.  Here, $H(\bmu)$ is an an entropy term which refers to the Shannon entropy of the graphical model with marginals $\bmu$.  While it may seem like this would be difficult to compute, it turns out to be particularly simple for Junction Trees.  In fact, it is a linear combination of local entropies and is known as the Kikuchi entropy (or Bethe entropy for pairwise models).  

\begin{equation} \label{eq:kikuchi}
H_{\kappa}(\bmu) = \sum_{r \in \C} \kappa_r H(\bmu_r)
\end{equation}

Above, $\kappa_r$ are the so-called overcounting numbers defined recursively by 

$$\kappa_r = 1 - \sum_{p \supset r} \kappa_p $$

This observation connecting exact marginal inference to this free energy minimization problem sparked an entire line of work on approximate inference algorithms that solve relaxations of this minimization problem.  Most notably is \emph{loopy belief propagation}, which applies the regular belief propagation updates on arbitrary factor graphs repeatedly until convergence.  The algorithm is well-defined for any factor graph, but it is only guaranteed to produce correct marginals for trees.   Nevertheless, it has often been observed to produce reasonable estimates in practice.  It turns out that if loopy belief propagation converges, the estimated marginals solve the following optimization problem:

\begin{equation} \label{eq:approx}
\bmu(\btheta) = \argmin_{\bmu \in \L} -\bmu^T \btheta - H_{\kappa}(\bmu)
\end{equation}

Above, $\L$ is the local polytope defined in \cref{eq:localpolytope}, and the exact entropy term is relaced with the approximation $H_{\kappa}$ (which is exact for trees).  This is a compelling property of loopy belief propagation that offers insight into its impressive performance in practice.  However, one main drawback of this approach is that loopy belief propagation is not guaranteed to convergence.  Moreover, if it does converge, it is not guranteed to be to a global minima of the free energy, as $-H_{\kappa}$ is not convex in general when $\kappa$ are the overcounting numbers.

Variants of loopy belief propagation have been proposed that optimize a ``convex free energy'' obtained by replacing the overcounting numbers $\kappa_r$ in the Kikuchi entropy with new values that lead to a convex entropy approximation.  It is known that $H_{\kappa}$ is convex (over the constraints) as long as the following condition is satisfied.  

$$ \sum_{r \in F(S)} \kappa_r \geq 0 $$

for all $S \subseteq \C$, where $F(S) = \set{r \in \C \mid \exists s \in S \text{ s.t. } r \subseteq s}$.  We are not aware of a message passing algorithm that can solve \cref{eq:approx} with arbitrary convex counting numbers.  However, if $\kappa_r > 0$ for all $r \in \C$, then several algorithms are applicable that are equipped with provable convergence guarantees.  Whether such an entropy approximation makes sense in terms of the quality of the approximation is not fully explored.  Typically, these convergent algorithms produce marginal estimates that are worse than those produced by loopy belief propagation, but since they are still valuable due to their compelling convergence guarantees.




%\begin{center}
%\begin{tabular}{ccc}
%Method & Limitations & Benefits \\\hline
%LBP & Factor graph (max overlap = 1) & Bethe entropy \\
%& not convex & \\\hline
%TRW & Pairwise factors & convex \\\hline
%Convex counting &  Factor graph (max overlap = 1) & convex \\
%& & any convex counting numbers \\\hline
%Generalized BP & not convex & Arbitrary graph \\
%& &  Kikuchi entropy \\\hline
%Convex GBP & Non-negative counting numbers & arbitrary graph \\
%& & convex \\\hline
%Unsolved & & Arbitrary graph \\
%& & convex \\
%& & Any convex counting numbers \\
%\end{tabular}
%\end{center}

%


==> methods.tex <==
\section{Use in Privacy Mechanisms} \label{sec:methods}

Next we describe how our estimation algorithms can improve the accuracy and/or scalability of four state-of-the-art mechanisms: MWEM, PrivBayes, HDMM, and DualQuery.

%\vspace{-1ex}
\textbf{MWEM.} The multiplicative weights exponential mechanism \cite{hardt2012simple} is an active-learning style algorithm that is designed to answer a workload of linear queries.  MWEM maintains an approximation of the data distribution and at each time step selects the worst approximated query $\q_i^T$ from the workload via the exponential mechanism \cite{mcsherry2007mechanism}. It then measures the query using the Laplace mechanism as $y_i = \q_i^T \p + z_i$ and then updates the approximate data distribution by incorporating the measured information using the multiplicative weights update rule.
%(either once, or iteratively).
The most basic version of MWEM represents the approximate data distribution in vector form, and updates it according to the following formula after each iteration:
%
%$$ \hat{\p} \leftarrow \hat{\p} \odot \exp{(\M_C^T (\M_C \hat{\p} - \y_C) / 2 m)} / Z $$
\begin{equation} \label{eq:mw}
\hat{\p} \leftarrow \hat{\p} \odot \exp{(-\q_i (\q_i^T \hat{\p} - y_i) / 2m)} / Z,
\end{equation}
%
where $\odot$ is elementwise multiplication and $Z$ is a normalization constant.  

It is infeasible to represent $\p$ explicitly for high-dimensional data, so this version of MWEM is only applicable to relatively low-dimensional data.  Hardt et al describe an enhanced version of MWEM, which we call \emph{factored MWEM}, that is able to avoid materializing this vector explicitly, in the special case when the measured queries decompose
%can be clustered into groups
over disjoint subsets of attributes.  
In that case, $\p$ is represented implicitly as a product of independent distributions over smaller domains, i.e., $\p(\x) = \prod_{C \in \C} \p_C(\x_C) $, and the update is done on one group at a time.
% on one of the clusters at a time
%However, this enhancement still breaks down for overlapping measurements on high-dimensional data, and so MWEM is still generally infeasible to run except on very simple workloads.
However, this enhancement breaks down for measurements on overlapping subsets of attributes in high-dimensional data, so MWEM is still generally infeasible to run except on simple workloads.

We can replace the multiplicative weights update with a call to Algorithm \ref{alg:proximal} using the standard $L_2$ loss function (on all measurements up to that point in the algorithm).  By doing so, we learn a compact graphical model representation of $\hat{\p}$, which avoids materializing the full $\p$ vector even when the measured queries overlap in complicated ways.  This allows MWEM to scale better and run in settings where it was previously infeasible. 
%
\revision{
Our efficient version of MWEM gives solutions that are identical to a commonly used MWEM variant. The MWEM update (Equation~\ref{eq:mw}) is closely related to the entropic mirror descent update \cite{beck2003mirror}, and, if iterated until convergence (as is done in practice), solves the same $L_2$ minimization problem that we consider. More details are given in Section ~\ref{sec:mw_emd} of the supplement.}

%\vspace{-1ex}
\textbf{PrivBayes.} PrivBayes \cite{zhang2017privbayes} is a differentially private mechanism that generates synthetic data.  It first spends half the privacy budget to learn a Bayesian network structure that captures the dependencies in the data, and then uses the remaining privacy budget to measure the statistics---which are marginals---necessary to learn the Bayesian network parameters.  PrivBayes uses a heuristic of truncating negative entries of noisy measurements and normalizing to get conditional probability tables. It then samples a synthetic dataset of $m$ records from the Bayesian network from which consistent answers to workload queries can be derived.  While this is simple and efficient, the heuristic does not properly account for measurement noise and sampling may introduce unnecessary error.
%it does not extract the most from the measured information which in turn hurts the accuracy.  

We can replace the PrivBayes estimation and sampling step with a call to Algorithm ~\ref{alg:proximal}, using an appropriate loss function (e.g. $L_1$ or $L_2$), to estimate a graphical model. 
%standard $L_2$ loss function
%\ds{Why $L_2$ specifically'? changed to ``an appropriate loss function''.}
Then we can answer new queries by performing graphical model inference (Section~\ref{inference}), rather than using synthetic data. 

%\ds{Try to be slightly more precise. Maybe something like: treat as the observations y within our framework, and then find a factored model p for answering future queries. Comment that when PrivBayes answers a query (as it will do in the next section) it will do so by sampling, while we will perform inference using the graphical model.}

%\ry{I think it another way to look at it is that privbayes estimation produces the synthetic data, and privbayes inference works directly over that tabular data.  As opposed to considering inference as sampling + query answering.  If we think about it this way, the output of estimation is some object that has an interface that allows you to answer queries (i.e., project, vectorize) which could be a contingency table, a tabular dataset, or a factored model.  While PrivBayes has two objects that support this interface (the bayesian network and the synthetic data), the final one is the synthetic database which is what we should consider for comparison purposes.}

%\vspace{-1ex}
\textbf{HDMM. } The high-dimensional matrix mechanism \cite{mckenna2018optimizing} is designed to answer a workload of linear queries on multi-dimensional data. It selects the measurements that minimize expected error on the input workload, which are then answered using the Laplace mechanism, and inconsistencies resolved by solving an ordinary least squares problem of the form:
%
$ \hat{\p} = \argmin \norm{ \Q \p - \y }_2 $.
%
Solving this least squares problem is the main bottleneck of HDMM, as it requires materializing the data vector even when $\Q$ contains queries over the marginals of $\p$.

We can replace the HDMM estimation procedure with  Algorithm~\ref{alg:proximal}, using the same $L_2$ loss function.  If the workload contains queries over low-dimensional marginals of $\p$, then $\Q$ will contain measurements over the low-dimensional marginals too.
Thus, we replace the full ``probability'' vector $\hat{\p}$ with a graphical model $\hat{\p}_{\btheta}$.
%The primary difference is that we find a non-negative $\p$ vector and we do it without materializing $\p$.
Also $\hat{\p}$ may contain negative values and need not sum to $1$ since HDMM solves an \emph{ordinary} (unconstrained) least squares problem.
%This improves the accuracy of HDMM and allows it to run in settings where it was previously infeasible to run. \ds{Last sentence seems more appropriate in results section?}
%\vspace{-1ex}

\textbf{DualQuery. } DualQuery \cite{Gaboardi14Dual} is an iterative algorithm inspired by the same two-player game underlying MWEM. It generates synthetic data to approximate the true data on a workload of linear queries.  DualQuery maintains a distribution over the workload queries that depends on the true data so that poorly approximated queries have higher probability mass.  In each iteration, samples are drawn from the query distribution, which are proven to be differentially private.  The sampled queries are then used to find a single record from the data domain (without accessing the protected data), which is added to the synthetic database.
%that explains the sample well, and it is added to the synthetic database.
%\ds{Description felt vague. I tried to make minor improvements. Still a bit vague, but maybe good enough?}

The measurements --- i.e., the random outcomes from the privacy mechanism --- are the queries sampled in each iteration.  Even though these are very different from the linear measurements we have primarily focused on, we can still express the log-likelihood as a function of $\p$ and select $\p$ to maximize the log-likelihood using Algorithm ~\ref{alg:proximal2} or \ref{alg:proximal}. The log-likelihood only depends on $\p$ through the answers to the workload queries. If the workload can be expressed in terms of $\bmu$ instead, the log-likelihood can as well.
%
Thus, after running DualQuery, we can call Algorithm \ref{alg:proximal2} with this custom loss function to estimate the data distribution, which we can use in place of the synthetic data produced by DualQuery.  The full details are given in the supplementary material.


==> my-approach.tex <==
\section{Our Approach}

In this section we describe our approach to overcome the main scalability limitations of \pgm, by introducing suitable approximations and new algorithmic techniques.  Our innovations allow us to scale significantly better than \pgm with respect to the size of $\C$. A high-level idea is to use approximate marginal inference in the \prox algorithm, but doing so naively makes it unclear what, if any, formal problem is being solved. We will develop a principled approach that uses approximate inference to \emph{exactly} solve a relaxed optimization problem.

\subsection{Region Graph}

\begin{figure}
  \begin{subfigure}[b]{0.19\textwidth}
    \centering\includegraphics[width=\textwidth]{fig/ex_clique}
    \caption{\label{fig:junction} Junction Tree}
  \end{subfigure}%
  \hspace{2em}
  \begin{subfigure}[b]{0.38\textwidth}
    \centering\includegraphics[width=\textwidth]{fig/ex_factor}
    \caption{\label{fig:factor} Factor Graph}
  \end{subfigure}%
  \hspace{2em}
  \begin{subfigure}[b]{0.38\textwidth}
    \centering\includegraphics[width=\textwidth]{fig/ex_region}
    \caption{\label{fig:region} Saturated Region Graph}
  \end{subfigure}%
\caption{\label{fig:regions} Comparison of different region graph structures defined over a domain with attributes $\set{A,B,C,D,E}$ that support the cliques $\C = \set{\set{A,B,C}, \set{A,D}, \set{B,C,D}, \set{D,E}}$.}
\end{figure}

Central to our approach is the notion of a \emph{region graph}.  A region graph is a data structure that (1) encodes constraints between subsets of attributes in a natural graphical format and (2) facilitates message passing algorithms for approximate marginal inference.


\begin{definition}[Region Graph]
A region graph $G = (\V, \E)$ is a directed graph where every vertex $r \in \V$ is an attribute clique and for any edge $r \rightarrow s \in \E$ we have that $ r \supseteq s $. We say that $G$ supports a clique set $\C$ if for every clique $r \in \C$, there exists some $r' \in \V$ such that $r \subseteq r'$.
\end{definition}
For any region graph, there is a corresponding set of constraints that characterize the \emph{local polytope} of internally consistent \emph{pseudo-marginals}, defined below.  

\begin{definition}[Local Polytope]
The local polytope of pseudo-marginals associated with a region graph $G$ is:
\begin{equation} \label{eq:localpolytope}
\L(G) =
  \left\{ \btau \geq 0
  \;\middle\vert\;
  \begin{array}{@{}l@{}l@{}}
  %\sum_{\x_r} \btau_r(\x_r) = 1 & \forall r \in \V \\
  %\sum_{\x_r \setminus \x_t} \btau_r(\x_r) = \btau_t(\x_t) \quad\quad & \forall r \rightarrow t \in \E\\
  \mathbf{1}^{\top} \btau_r = 1 & \forall r \in \V \\
  P_{r \rightarrow s} \btau_r = \btau_s \quad \quad & \forall r \rightarrow s \in \E \\
  \end{array}
  \right\}.
\end{equation}
\end{definition}

The general idea is to relax problems involving the intractable marginal polytope to use the local polytope instead, since $\M(\V) \subseteq \L(G)$ and $\L(G)$ is straightforward to representat using the linear constraints in Eq.~\eqref{eq:localpolytope}.  We use the notation $\btau$ in place of $\btau$ to emphasize that $\btau$ is not necessarily a valid marginal vector, even though we will generally treat it as such.  This notational choice is standard in the graphical models literature \cite{wainwright2008graphical}.

The nodes and edges in the region graph dictate which constraints we expect to hold among pseudo-marginals.  As discussed  below, region graphs can encode junction trees and factor graphs as special cases.  
%
For example, \cref{fig:regions} shows three different region graphs that support $\C = \set{\set{A,B,C}, \set{A,D}, \set{B,C,D}, \set{D,E}}$.  At one extreme is the \textbf{Junction Tree}, shown in \cref{fig:junction}, which is obtained by merging cliques \set{A,B,C}, \set{A,D}, and \set{B,C,D} into a super-clique $\set{A,B,C,D}$. This region graph structure exactly encodes the marginal polytope, that is, $\L(G) \equiv \M(\V)$. Ordinary belief propagation in this graph corresponds to exact marginal inference.  At the other end of the extreme is the \textbf{Factor Graph}, shown in \cref{fig:factor}.  This graph contains one vertex for every clique $r \in \C$, plus additional vertices for the singleton cliques.  It encodes constraints that all cliques must agree on common one-way marginals. For example, $\btau_{ABC}$ and $\btau_{BCD}$ must agree on the shared one-way marginals $\btau_B$ and $\btau_C$, but not necessarily on the shared two-way marginal $\btau_{BC}$.  A natural middle ground is the fully \textbf{Saturated Region Graph}, shown in \cref{fig:region}.  This graph includes every clique $r \in \C$ as a vertex, and includes additional vertices to capture intersections between those cliques.  Unlike the factor graph, this graph does require that $\btau_{ABC}$ is consistent with $\btau_{BCD}$ with respect to the $\btau_{BC}$ marginal.  Unlike the junction tree, this graph does not require forming super-cliques whose size grow quickly with $|\C|$.  For more details about the concepts above, please refer to \cite{koller2009probabilistic}.
%\ds{Give citations for facts and background concepts in this pargraph that are not fully explained or supported, e.g., junction tree, saturated region graph. A blanket citation might work, but targeted could be better.} \ry{agree targeted is nice, but I think I would just cite Koller and Friedman for all of these.}


The methods we describe in this paper apply for any region graph that supports $\C$.
By default, we simply use the fully saturated region graph, which can easily be constructed given the cliques $\C$ \cite{koller2009probabilistic}.

\begin{definition}[Saturated Region Graph]
Given a set of cliques $\C$, the associated saturated region graph is constructed as follows:\ry{TODO}
\begin{enumerate}
\item $\C \subseteq \V$
\item $\V$ is closed under intersection
\item Whenever $r \supseteq s $ and there is no $t$ such that $ r \supseteq t \supseteq s$, there is an edge $r \rightarrow s$.  
\item cliques in $\C$ do not have parents (or if they do, parents are also in $\C$)
\end{enumerate}
\end{definition}

%% \ds{Orphaned:} For a graphical model $\p_\btheta$ on clique set $\C$ and a region graph that supports $\C$, the goal is to estimate the marginal distributions associated with each vertex in the graph, i.e., $\btau = (\btau_r)_{r \in V}$. Since $G$ supports $\C$, we can easily compute $(\btau_r)_{r \in \C}$ from $(\btau_r)_{r \in V}$ via marginalization, so this solves our original inference goal of estimating $\M_\C \p_\btheta$. Additionally, we can optimize any function over $\M(\C)$ by optimizing an equivalent function over $M(\V)$.\footnote{Let $P$ be the marginalization operation to compute $\btau_r$ from $\btau_{r'}$ for some $r' \in \V$ for each $r \in \C$. $P$ is linear and maps $\M(\V)$ onto $\M(\C$), therefore $\min_{\btau \in \M(\C)} L(\btau) = \min_{\btau' \in \M(\V)}L'(\btau')$ for $L'(\btau') = L(P\btau')$.}

\subsection{Estimation: Finding an Approximate Data Distribution Representation} \ry{may have to change title; where is the data distribution?}

We begin by introducing a very natural relaxation of the problem we seek to solve.

\begin{problem}[Convex Optimization over the Local Polytope] \label{prob:convex}
Given a region graph $G$ and a convex loss function $L(\btau)$ where $\btau = (\btau_r)_{r \in V}$, solve:
%
$$ \hat{\btau} = \argmin_{\btau \in \L(G)} L(\btau). $$ 
\end{problem}

In the problem above, we simply replaced the marginal polytope $\M(\V)$ from our original problem\footnote{If $G$ supports $\C$, we can assume without loss of generality that \cref{prob:marginal} was defined on $\M(\V)$ instead of $\M(\C)$. In particular, the loss function $L$ can be written to depend on marginals $(\btau_{r'})_{r' \in \V}$ instead of $(\btau_r)_{r \in \C}$, because the latter can be computed from the former.} with the local polytope $\L(G)$. Since this is a convex optimization problem with linear constraints, it can be solved with a number of general purpose techniques, including interior point and active set methods \cite{boyd2004convex}.  However, these methods do nothing to exploit the special structure in the constraint set $\L(G)$, and as such, they have trouble running on large-scale problems.  

Our first contribution is to show that we can solve \cref{prob:convex} efficiently by instantiating \prox with a carefully chosen approximate marginal oracle.  To do so, it is useful to view the problem of approximate marginal inference through the lens of the free energy minimization problem, stated below.

\begin{problem}[Approximate Free Energy Minimization] \label{prob:energy}
Let $G=(\V,\E)$ be a region graph, $\btheta = (\btheta_r)_{r \in \V}$ be real-valued parameters, and $H_{\kappa}(\btau) = \sum_{r \in \V} \kappa_r H(\btau_r) $, where $\kappa_r \in \mathbb{R}$ are counting numbers, and $H(\btau_r) = -\sum_{\x_r \in \dom_r} \btau_r(\x_r) \log{\btau_r(\x_r)}$ is the Shannon entropy of $\btau_r$.
%
$$ \hat{\btau} = \argmin_{\btau \in \L(G)} -\btau^{\top} \btheta - H_{\kappa}(\btau) $$
\end{problem}

This problem approximates the (intractable) variational free energy minimization problem~\cite{wainwright2008graphical}, for which the optimum gives the true marginals of $\p_\btheta$, by using $\L(G)$ instead of $\M(\V)$, and using $H_{\kappa}(\btau)$ as an approximation to the full Shannon entropy.
%\ds{TODO: add sentence here to connect to exact inference} If $G$ is a Junction Tree, and the counting numbers $\counting$ are chosen appropriately, then it can be shown that the marginals of the graphical model with parameters $\btheta$ exactly solve \cref{prob:energy}.
Many algorithms for approximate marginal inference can be seen as solving variants of this free energy minimization problem under different assumptions about $G$ and $\counting$ \cite{heskes2004uniqueness,wainwright2003tree,wiegerinck2005approximations,loh2014concavity,hazan2012tightening,yedidia2005constructing,hazan2012convergent,meltzer2012convergent,heskes2006convexity,heskes2003generalized,pakzad2005estimation}.  %\ds{The rest of this paragraph has background that may not be needed. Consider dropping parts about Bethe and loopy BP especially, maybe also TRW. Add citations for statements like ``many algorithms can be seen as...''} Indeed, one of the most famous approximate inference algorithms, \emph{loopy belief propagation} on a factor graph, falls into this category.  In particular, if loopy belief propagation converges, it converges to a fixed point of \cref{prob:energy}, where $\counting$ correspond to the Bethe-entropy approximation.  Unfortunately, the Bethe entropy is not convex except in special cases, and loopy belief propagation is not guaranteed to converge in general.  For this reason, variants of loopy belief propagation have been proposed that can be shown to solve \cref{prob:energy} where $\counting$ are \emph{convex} counting numbers (i.e., they correspond to a convex entropy approximation).  One well-known algorithm from this class is tree-reweighted belief propagation \cite{wainwright2003tree}.  However, this algorithm is only applicable for pairwise models (i.e., $|r| \leq 2$ for all $ r \in V$).  A more general but lesser-known algorithm was proposed by Hazan et al. \cite{hazan2012tightening} and is shown in \cref{alg:mpconvex}.  Other related algorithms for this problem also exist \cite{wiegerinck2005approximations,loh2014concavity}. 

\begin{theorem}[Algorithm for Approximate Free Energy Minimization \cite{hazan2012tightening}] \label{thm:energy}
Given a region graph $G$, parameters $\btheta = (\btheta_r)_{r \in \V}$, and any positive counting numbers $\counting_r > 0$ for $ r \in \V$, \gbp solves the approximate free energy minimization problem of \cref{prob:energy}.  
\end{theorem}

Importantly, the complexity of \cref{alg:mpconvex} depends mainly on the size of the largest clique in the region graph.  In many cases of practical interest, this will be exponentially smaller in the saturated region graph than in a junction tree. %\ds{Suggest jumping straight from here to Theorem.} %One limitation of \cref{alg:mpconvex} is that its correctness depends on every counting number being positive.  This is somewhat unnatural, because when $G$ is a junction tree, exact marginal inference solves \cref{prob:energy} with positive and negative counting numbers.  Hence, \cref{alg:mpconvex} does not reduce to ordinary belief propagation when $G$ is a junction tree.  Remarkably, this drawback will not matter for our purposes, as we show in \cref{thm:approx}  

\begin{theorem} \label{thm:approx}
When \prox uses \gbp as the \oracle (with \textbf{any} positive counting numbers $\kappa$), it solves the convex optimization problem over the local polytope of \cref{prob:convex}.
\end{theorem}

This result is remarkable in light of previous work, where different counting number schemes are used with the goal of tightly approximating the true entropy, and form the basis for different approximate inference methods. In our setting, all methods with \emph{convex} counting numbers are equivalent: they may lead to different \emph{parameters} $\hat\btheta$, but the corresponding pseudo-marginals $\hat\btau = \gbp(\hat\btheta)$ are invariant. Indeed, the optimal $\hat\btau$ depends only on the estimation objective $L(\btau)$ and the structure of the local polytope. We conjecture that a similar invariance holds for traditional marginal-based learning objectives with approximate inference~\cite{domke2013learning} when message-passing algorithms based on convex free-energy approximations are used as the approximate inference method.

\begin{proof}
Since $L$ is a convex function and $\L$ is a convex constraint set, this problem can be solved with mirror descent \cite{beck2003mirror}.  Each iteration of mirror descent requires solving subproblems of the form:
%
$$\btau^{t+1} = \argmin_{\btau \in \L(G)} \btau^{\top} \grad L(\btau^t) + \frac{1}{\eta_t} D(\btau, \btau^t) \quad\quad D(\btau, \btau^t) = \psi(\btau) - \psi(\btau^t) - (\btau - \btau^t)^{\top} \grad \psi(\btau^t)$$
%
Here, $D$ is a Bregman distance measure and $\psi$ is some strongly convex and continuously differentiable function.  Setting $ \psi = -H_{\counting}$, a negative weighted entropy with any (strongly) convex counting numbers $\counting$, we arrive at the following update equation:
%
\begin{align*}
%\btau^{t+1} &= \argmin_{\btau \in \L} \btau^{\top} \grad L(\btau^t) + \frac{1}{\eta_t} D(\btau, \btau^t) \\
\btau^{t+1} &= \argmin_{\btau \in \L(G)} \btau^{\top} \grad L(\btau^t) + \frac{1}{\eta_t} \Big( -H(\btau) + H(\btau^t) + (\btau - \btau^t)^{\top} \grad H_{\counting}(\btau^t) \Big) \\
%&= \argmin_{\btau \in \L} \btau^{\top} \grad L(\btau^t) + \frac{1}{\eta_t} \Big( -H_{\rho}(\btau) + \btau^T \grad H_{\rho}(\btau^t) \Big) \\
%&= \argmin_{\btau \in \L} \btau^{\top} \Big(\grad L(\btau^t) + \frac{1}{\eta_t} \grad H_{\rho}(\btau^t) \Big) - \frac{1}{\eta_t} H_{\rho}(\btau) \\
&= \argmin_{\btau \in \L(G)} \btau^{\top} \Big(\eta_t \grad L(\btau^t) + \grad H_{\counting}(\btau^t) \Big) - H_{\counting}(\btau) \tag{algebraic manipulation} \\
&= \argmin_{\btau \in \L(G)} \btau^{\top} \Big(\eta_t \grad L(\btau^t) - \btheta^t \Big) - H_{\counting}(\btau) \tag{\cref{thm:cvxdual}; Supplement} \\
%&= \btau \big( -\eta_t \grad L(\btau^t) - \grad H(\btau^t) \big) \\
&= \gbp \big(G, \btheta^t -\eta_t \grad L(\btau^t), \counting \big) \tag{\cref{thm:energy}}
\end{align*}
%
\end{proof}

\begin{algorithm}
%\caption{Message Passing for Convex Free Energy on a Region Graph \cite{hazan2012tightening}} \label{alg:mpconvex}
\caption{\gbp \cite{hazan2012tightening}} \label{alg:mpconvex}
\begin{algorithmic}
\STATE {\bfseries Input:} Region Graph $G=(\V,\E)$, parameters $\btheta = (\btheta_r)_{r \in \V}$, convex counting numbers $\counting_r > 0$
\STATE {\bfseries Output:} Pseudo-marginals $\btau = (\btau_r)_{r \in \C}$
\STATE $\counting_{r,t} = \counting_r / (\counting_t + \sum_{p \rightarrow t} \counting_p)$
\STATE Initialize $m_{r\rightarrow t}(\x_t) = 0$ and $\lambda_{t \rightarrow r}(\x_t) = 0$
\FOR{$i = 1,\dots$}
\FOR{$r \rightarrow t \in \E$}
\STATE $m_{r \rightarrow t}(\x_t) = \counting_r \log{\Big( \sum_{\x_r \setminus \x_t} \exp{\Big( (\btheta_r(\x_r) + \sum_{c \neq r} \lambda_{c \rightarrow r}(\x_c) - \sum_{p} \lambda_{r \rightarrow p}}(\x_p))/\counting_r)\Big)\Big)}$
\STATE $\lambda_{t \rightarrow r}(\x_t) = \counting_{r,t} \Big( \btheta_t(\x_t) + \sum_{c} \lambda_{c \rightarrow t}(\x_t) + \sum_{p} m_{p \rightarrow t}(\x_t) \Big) - m_{t \rightarrow r}(\x_t)$
\ENDFOR
\ENDFOR
\FOR{$r \in \V$}
\STATE $\btau_r(\x_r) \propto \exp{\Big((\btheta_r(\x_r) + \sum_{t} \lambda_{t \rightarrow r}(\x_t) - \sum_p \lambda_{r \rightarrow p}(\x_r))/\counting_r\Big)}$
\ENDFOR
\RETURN $\btau = (\btau_r)_{r \in \V}$
\end{algorithmic}
\end{algorithm}


\subsection{Inference: Answering New Queries}

We now turn our attention to the problem of inference.  The central challenge is to estimate out-of-clique marginals.  That is, we want to estimate $\btau_r$ where $r \not \in \C$.  Previously, we accomplished this by computing the marginal of $\p_{\btheta}$. Unfortunately, that approach no longer makes sense here, because (1) variable elimination in $\p_{\btheta}$ is intractable for the class of models we are interested in, and (2) even if it was tractable, it would give the ``wrong'' answer, since the true marginals of the graphical model with parameter $\btheta$ will be different from the ones estimated in \prox (in this case, the true marginals are not the correct ones), and the difference may be substantial for some choices of convex counting numbers $\counting$.

We thus propose two different methods that do not have these drawbacks, and discuss their benefits and drawbacks.  We expand on this discussion, and consider even more alternatives in the supplement.   

\textbf{Running \prox over an expanded region graph.}  Recall that \prox solves \cref{prob:convex} for \emph{any} region graph that supports $\C$ \footnote{note that the problem itself is slightly different for different region graphs, because the definition of the local polytope depends on the choice of region graph.}.  By default, we use the saturated region graph of $\C$, which is in some sense the smallest graph that encodes all internal consistency constraints.  However, we can expand this region graph to include new vertices and edges corresponding to the cliques whose marginals we want to estimate, even if the loss function does not depend on those marginals.  Clearly, the new region graph is still valid, and \gbp over this graph will return all desired marginals.

The additional cliques do not affect the loss function (the gradient and log-potentials will always remain $\mathbf{0}$ for the new cliques), but they do impact the constraints.  Upon convergence, the estimated pseudo-marginals will belong to the local polytope of the expanded region graph, and hence they will all be locally consistent.  

However, this approach comes at a potentially high cost, since the region graph contains more vertices and edges, each iteration of \prox requires more time, and the algorithm as a whole is slower than it otherwise would be.   This can be especially potent if we wanted to estimate all 3-way marginals, and only measured 10 of them.  This approach adds a significant number of vertices and edges to the region graph, and substantially slows down \gbp and consequently \prox as well.

\textbf{Minimizing Constraint Violation and Maximizing Entropy}
In light of the drawback of the previous approach, we propose a new method which does not require running \prox over a larger region graph.  This approach is a simple post-processing of the output of \prox run over the original region graph, and it can be easily parallelized as well.  For a given clique $r \not \in \V_+$, we would like choose $\btau_r$ to (1) be internally consistent with the existing pseudo-marginals $\btau$ and (2) to maximize entropy among all internally consistent choices.  However, it is certainly possible that there are \emph{no} choices of $\btau_r$ that are internally consistent with $\btau$ (see Example 4.1 in \cite{wainwright2008graphical}).  Thus, we propose the following instead: (1) choose $\btau_r$ to minimize some natural quantification of the constraint violation, and (2) among choices that minimize this quantity, select the one with maximum entropy.  We begin by formalizing the first problem, and then discuss our solution to it, which solves the second problem ``for free''.

\begin{problem}[Minimizing Constraint Violation] \label{prob:project}
Let $\btau$ be a vector of pseudo-marginals defined over cliques $\V$ and let $ \C' $ be a collection of new cliques.  For each $ r \in \C'$,
$$ \btau'_r = \argmin_{\btau_r \in \S} \sum_{t,s \in \mathcal{B}} \norm{P_{r \rightarrow s} \btau_r - P_{t \rightarrow s} \btau_s}_2^2 $$
where $\S = \set{ \btau_r \geq 0 \mid \mathbf{1}^{\top} \btau_r = 1}$ is the probability simplex, and $\mathcal{B} = \set{(t, t \cap r) \mid t \in \V}$.
\end{problem}


This is a quadratic minimization problem over the probability simplex.  It can be readily solved with iterative proximal algorithms like entropic mirror descent \cite{beck2003mirror}.   Entropic mirror descent guarantees the solution found will have maximum entropy among all minimizers of the objective.  Additionally, this method does not require any information about attributes not in $r$, and even though it is an iterative algorithm, each iteration runs much faster than an iteration of $\gbp$.  Additionally, if we want to estimate many new marginals, each one can be done in parallel, as the optimization problems do not depend on each other.

However, unlike the first approach of expanding the region graph, this one does not guarantee internal consistency between the existing pseudo-marginals and the new ones.  We generally expect the first method to give slightly better results, at the cost of increased computation.  In general, we expect the second method to perform nearly as well, and run much faster.  

We discuss the problem of inference to out-of-clique marginals in greater detail in the supplement, including additional approaches and special cases not covered here.


==> technical.tex <==
\section{Algorithms for Estimation and Inference}\label{approach}

%\ry{TODO: differing noise scales}

%\subsection{Optimization for Estimation}\label{optimization-for-estimation}

%We observe \(\y\) (as defined above) and want to answer a target query \(\q\). (For now assume we are answering just one \ryref{arbitrary test query}{note: representing an arbitrary query may be intractable in the worst case}.  Later we will discuss answering many queries or queries with more structure.) We either didn't ask \(\q\) directly, or we did ask it but want to use \emph{all} of the available information to estimate \(\q^T \p\) as opposed to just using the noisy answer we got.

What principle can we follow to estimate answers to the workload query set? Prior work takes the approach of first using all available information to estimate a full contingency table \(\hat{\p} \approx \p\) and then using \(\hat{\p}\) to answer later queries~\cite{hay2010boosting,li2010optimizing,ding2011differentially,qardaji2013understanding,lee2015maximum}.
%The most common approach to estimating $\p$ is to solve a least squares problem of the form: $$ \hat{\p} = \argmin_{\p} || \Q \p - \y ||_2 $$, and many differentially private mechanisms solve a problem of this form using special-purpose techniques.  
We will call finding \(\hat{\p}\) \emph{estimation}, and using \(\hat{\p}\) to answer new queries \emph{inference}.
%which will match more closely terminology used in probabilistic modeling.

\subsection{Optimization Formulation} \label{sec:formulation}
%\ds{I could imagine a rewrite of this section that is entirely based on the log-likelihood... but I think it's not worth it at this stage.}
%We focus on the more standard case of linear queries. The standard optimization framework for estimation and inference in this case is:
The standard framework for estimation and inference is:
\begin{align*}
\hat{\p} &\in \argmin_{\p \in \mathcal{S}} L(\p), & \text{(estimation)} \\
f_{\W}(\db) &\approx \W\, \hat{\p}. &\text{(inference)}
\end{align*}
Here $ \mathcal{S} = \big\{ \p: \p \geq 0, \mathbf{1}^T \p = 1\big\} $  is the probability simplex and $L(\p)$ is a loss function that measures how well $\p$ explains the observed measurements. In past works, $L(\p) = \norm{ \Q \p - \y }$ has been used as a loss function, where $\Q$ is the measured query set and $ \norm{ \cdot } $ is either the $L_1$ norm or $L_2$ norm.  Minimizing the $L_1$ norm is equivalent to maximum likelihood estimation when the noise comes from the Laplace mechanism~\cite{lee2015maximum}.
%entries of the noise vector are sampled iid from a Laplace distribution \cite{lee2015maximum}.
Minimizing the $L_2$ norm is far more common in the literature however, and it is also the maximum likelihood estimator for Gaussian noise \cite{hay2010boosting,Nikolov13Geometry,li2014data,qardaji2013understanding,ding2011differentially,Xiao10Differential,li2010optimizing, mckenna2018optimizing}. Our method supports both of these loss functions; we only require that $L$ is convex. Both of these loss functions are easily adapted to the situation where queries in $\Q$ may be measured with differing degrees of noise.
The constraint $\p \in \mathcal{S}$ may also be relaxed, which simplifies $L_2$ minimization; additionally, under different assumptions and an alternate version of privacy, the number of individuals may not be known.
%Sometimes the constraint $ \p \in S $ is relaxed so that the entries of $\p$ may be positive or negative, and they need not sum exactly to $m$.  
%
All existing algorithms to solve these variations of the estimation problem suffer from the same problem: they do not scale to high dimensions since the size of $\p$ is exponential in $d$ and we have to construct it explicitly as an intermediate step even if the inputs and outputs are small (e.g., all measurement queries are over low-dimensional marginals).  


%\textbf{Problem}: this doesn't scale to high dimensions. The size of `\(\p\) is exponential in \(d\), and we have to construct it as an intermediate step even if the inputs and outputs are small, e.g., if all measurement queries and the target query are low-dimensional. (This really happens.)

\textbf{Optimization in Terms of Marginals.}\label{optimization-in-terms-of-marginals}
For marginal query sets, a loss function will typically depend on $\p$ only through its marginals $\bmu$. For example, when $\Q = \Q_\C \M_\C$ we have $L(\p) = \| \Q\p - \y \| = \| \Q_\C \bmu - \y\| = L(\bmu)$ where we now write the loss function as $L(\bmu)$. More generally, we will consider \emph{any} loss function that only depends on the marginals. A very general case is when $L(\bmu) = -\log p(\y \mid \bmu)$ is the negative log-likelihood of \emph{any} differentially private algorithm that produces output $\y$ that depends only on the marginal vector $\bmu$ (see our treatment of DualQuery\eat{, \citeauthor{Gaboardi14Dual}, \citeyear{Gaboardi14Dual},} in Section~\ref{sec:methods}).% This extension also allows linear queries that are ``non-local'' in the sense of~\cite{vilnis2015bethe}: they depend on many variables but only through the marginals $\bmu$, e.g., a sum over many marginals.}
%For example, when all the measurements are taken with respect to the concatenated vector of marginals, the loss can be expressed as $L(\bmu) = || \Q \bmu - \y || $

The marginal vector $\bmu$ may be much lower dimensional than $\p$. How can we take advantage of this fact? An ``obvious'' idea would be to modify the optimization to estimate only the marginals as $\hat{\bmu} \in \argmin_{\bmu \in \marg} L(\bmu)$, where \(\marg = \big\{ \bmu: \exists \p \in \mathcal{S} \text{ s.t. } \M_\C \p = \bmu\}\) is the marginal polytope, which is the set of all valid marginals. There are two issues here. First, the marginal polytope has a complex combinatorial structure, and, although it is a convex set, it is generally not possible to enumerate its constraints for use with standard convex optimization algorithms. Note that this optimization problem is in fact a \emph{generic} convex optimization problem over the marginal polytope, and as such it generalizes standard graphical model inference problems~\cite{wainwright2008graphical}. Second, after finding $\hat{\bmu}$ it is not clear how to answer new queries, unless they depend only on some measured marginal \(\bmu_C\).

%\ry{should we also say something about the difficulty of solving a constrained optimiztion problem over the marginal polytope?  Or is that a moot point for this audience?}

% I no longer think the next statements are relevant / appropriate.
%Second, even for queries that are determined by a measurement marginal \(\bmu_C\), it is unclear what criterion is being used to answer the query.
% For example, the constraint set implies that \emph{some} information from other cliques is being used to estimate \(\bmu_C\), but how, exactly, is this information ``transferred'' to the estimate \(\hat{\bmu}_C\)?


%\textbf{Factored \(\p\) and Maximum Entropy Criterion.}
\textbf{Graphical Model Representation.}
\label{factored-p-and-maximum-entropy-criterion}
After finding an optimal $\hat{\bmu}$ we want to answer new queries that do not necessarily depend directly on the measured marginals.  To do this we need to identify a distribution $\hat{\p}$ that has marginals $\hat{\bmu}$, and we must have a tractable representation of this distribution.  Also, since there may be many $\hat{\p}$ that give rise to the same marginals, we want a principled criteria to choose a single estimate, such as the principle of maximum entropy.  We accomplish these goals using undirected graphical models. 

\eat{
\revision{Informally, a graphical model is a factored representation of a distribution that avoids storing an entry for every element of the domain.  It is parameterized by a vector of potentials $\btheta$, which is typically much smaller than the size of the domain.  For more background on graphical models, refer to \cite{koller2009probabilistic} and \cite{wainwright2008graphical}.}
}

\revision{A graphical model represents a high-dimensional distribution as a product
 of factors $\boldsymbol{\phi}_C$ defined on attribute subsets, i.e., $\p(\x)= \prod_{C \in \mathcal{C}}\boldsymbol{\phi}_C(\x_C)$. A factored representation is often much more compact than an explicit one and facilitates efficient computation of marginals~\cite{koller2009probabilistic}. We use a log-linear form with parameters $\btheta_C(\x_C) = \log \boldsymbol{\phi}_C(\x_C)$.}


% This paragraph is repetitive with the two formal statement below, so I deleted it
%
%We will show that, given a solution \(\hat{\bmu} \in \argmin_{\bmu \in \marg} L(\bmu)\), we can find a factored distribution \(\hat{\p}\) that has maximum entropy among all distributions with marginals \(\hat{\bmu}\). Because it is factored, we can represent \(\hat{\p}\) compactly and use it to answer new queries efficeintly.  This solves both of our problems.  The factorization is chosen based on the measurement queries (not the other way around, as in Bernstein et al. \cite{bernstein2017differentially}) and this imposed structure on the distribution does not prevent us from finding a solution that minimizes the loss globally.

\begin{definition}[Graphical model]
  Let \(\p_{\btheta}(\x) = \frac{1}{Z} \exp \big(\sum_{C \in \C} \btheta_C(\x_C) \big)\) be a normalized distribution, where $\btheta_C \in \R^{n_C}$. This distribution is a graphical model that factors over the measurement sets \(\C\), which are the cliques of the graphical model. The vector \(\btheta = (\btheta_C)_{C \in \C}\) is the parameter vector.
  \label{def:graphical-model}
\end{definition}

\begin{theorem}[Maximum entropy \cite{wainwright2008graphical}] \label{theorem:maxent} %\ry{better name, more precise}
  Given any $\hat{\bmu}$ in the interior of $\marg$ there is a parameter vector \(\hat{\btheta}\) such that the graphical model \(\p_{\hat{\btheta}}(\x)\) has maximum entropy among all $\hat{\p}(\x)$
with marginals \(\hat{\bmu}\).\footnote{If the marginals are on the boundary of $\marg$, e.g., if they contain zeros, there is a sequence of parameters $\{\btheta^{(n)}\}$ such that $\p_{\btheta^{(n)}}(\x)$ converges to the maximum-entropy distribution
    %with marginals $\hat{\bmu}$
    as $n \to \infty$. See~\cite{wainwright2008graphical}.
    %The marginals will belong to the boundary of $\marg$ if they contain zeros.
  }
 %The parameters are not uniquely determined by \(\hat{\bmu}\) but the maximum entropy distribution \(\p(\x; \hat{\btheta}(\hat{\bmu}))\) is unique.
\end{theorem}
Theorem~\ref{theorem:maxent} says that, after finding $\hat{\bmu}$, we can obtain a factored representation of the maximum-entropy distribution with these marginals by finding the graphical model parameters $\hat{\btheta}$. % that characterize the distribution $\hat{\p}$
This is the problem of learning in an graphical model, which is well understood~\cite{wainwright2008graphical}.

%Theorem~\ref{theorem:maxent} comes directly from the Wainwright and Jordan text (theorem 3.4) \cite{?}. \ry{what if $\bmu$ has zeros?}

%\textbf{Technical notes}
%\begin{itemize}
%\item
%  As stated this is basically a direct consequence of standard marginal
%  polytope stuff from Wainwright and Jordan (Theorem 3.4 and surrounding
%  content)
%\item
%  There is a technicality: the theorem as stated only applies if
%  \(\hat{\bmu}\) is in the \emph{interior} of the marginal polytope.
%  Specifically this means it has no zeros. We need to figure out what to
%  say if \(\hat{\bmu}\) has zeros. I hope there will be a satisfactory
%  precise statement. Something like: there is a sequence of
%  values\ldots{} (see part (a) of Theorem 3.4).
%\item
%  \textbf{Ideally we'd like a stronger statement}: we can find a
%  factored distribution that has maximum entropy among all distributions
%  with marginals that minimize \(L(\bmu)\). Mathematically it would look
%  something like this: \[
%    \p(\x; \hat{\btheta}) \in \argmax_{\p \in \mathcal{S}} H(\p) \quad \text{s.t. } \, \bmu(\p) \in \argmin_{\bmu \in \marg} L(\bmu)
%    \] The reason we don't obviously get this is because if \(L(\bmu)\)
%  has multiple minima, we might choose one minimum \(\hat{\bmu}\) that
%  leads to lower entropy than if we had chosen a different one. If
%  \(L(\bmu)\) is strictly convex, it has a single minimum and we get
%  what we want. There's a chance that we get the stronger property
%  defined by the way we solve the problem (e.g., the proximal method)
%  but this is something we'd have to analyze much more carefully.
%\item
%  TODO: Dan come back and resolve as much of this as possible. Ryan,
%  feel free to take a crack at it if you want.
%\end{itemize}
%

\subsection{Estimation: optimizing over the marginal polytope}\label{estimation}

\setlength{\textfloatsep}{15pt}
\begin{algorithm}[tb]
    \caption{Proximal Estimation Algorithm} \label{alg:proximal2}
\begin{algorithmic}
    \STATE {\bfseries Input:} Loss function $L(\bmu)$ between $\bmu$ and $\y$
    \STATE {\bfseries Output:} Estimated data distribution $\hat{\p}_{\btheta}$
    \STATE $\btheta = \vect{0}$
    \FOR{$t=1, \dots, T$}
        \STATE $\bmu = \oracle(\btheta)$
        \STATE $\btheta = \btheta - \eta_t \grad L(\bmu)$
    \ENDFOR
    \STATE {\bfseries return} $\hat{\p}_{\btheta}$
\end{algorithmic}
\end{algorithm}

We need algorithms to find \(\hat{\bmu}\) and \(\hat{\btheta}\).  We considered a variety of algorithms and present two of them here.  Both are proximal algorithms for solving convex problems with ``simple'' constraints \cite{parikh2014proximal}.  Central to our algorithms is a subroutine \oracle{}, which is some black-box algorithm for computing the clique marginals $\bmu$ of a graphical model from the parameters $\btheta$.  This is the problem of \emph{marginal inference} in a graphical model.  \oracle{} may be any marginal inference routine --- we use belief propagation on a junction tree. In the remainder of this section, we assume that the clique set $\C$ are the cliques of a junction tree. This is without loss of generality, since we can enlarge cliques as needed until this property is satisfied.

Algorithm~\ref{alg:proximal2} is a routine to find $\hat{\bmu}$ by solving a convex optimization problem over the marginal polytope. Due to the special structure of the algorithm it also finds the parameters $\hat{\btheta}$. Algorithm~\ref{alg:proximal2} is inspired by the entropic mirror descent algorithm for solving convex optimization problems over the probability simplex \cite{beck2003mirror}.  The iterates of the optimization are obtained by solving simpler optimization problems of the form: \vspace{-1ex}
%
\begin{equation} \label{eq:update}
\bmu^{t+1} = \argmin_{\bmu \in \marg} \bmu^T \grad L(\bmu^t) + \frac{1}{\eta_t} D(\bmu, \bmu^t)
\end{equation}
%
where $D$ is a Bregman divergence that is chosen to reflect the geometry of the marginal polytope.  Here we use the following Bregman divergence generated from the Shannon entropy: $ D(\bmu, \bmu^t) = -H(\bmu) + H(\bmu^t) + (\bmu - \bmu^t)^T \grad H(\bmu^t) $, where $H(\bmu)$ is the Shannon entropy of the graphical model $\p_{\btheta}$ with marginals $\bmu$. Since we assumed above that $\bmu$ are marginals of the cliques of a junction tree, the Shannon entropy is convex and easily computed  as a function of $\bmu$ alone~\cite{wainwright2008graphical}.\footnote{An alternative would be to use the Bethe entropy as in ~\cite{vilnis2015bethe}. The Bethe entropy is convex and computable from $\bmu$ alone regardless of the model structure. Using Bethe entropy would lead to approximate marginal inference instead of exact marginal inference as the subproblems, which is an interesting direction for future work.}

%\ds{need to be careful here about Bethe entropy}
%
%\ds{It's only true that Bethe entropy = Shannon entropy on trees. Bethe entropy is usually thought of as a computationally tractable approximation of the Shannon entropy. So it's confusing to conflate them like this. I believe you are always doing exact inference using a junction tree, in which case they coincide. Let's talk about which term you should use. I think it needs to be Bethe entropy because this is always convex in mu. Otherwise we have to assume the model is tree-structured or formulate the algorithm differently.}
%
With this divergence, the objective of the subproblem in Equation \ref{eq:update} can be seen to be equal to a variational free energy, which is minimized by marginal inference in a graphical model.
%Thus, the subproblem can be solved by \oracle{}.
The full derivation is provided in the supplement.  The implementation of Algorithm \ref{alg:proximal2} is very simple --- it simply requires calling \oracle{} at each iteration.  Additionally, even though the algorithm is designed to find the optimal $\bmu$, it also returns the corresponding graphical model parameters $\btheta$ ``for free'' as a by-product of the optimization.  This is evident from Algorithm \ref{alg:proximal2}: upon convergence, $\bmu$ is the vector of marginals of the graphical model with parameters $\btheta$. The variable $\eta_t$ in this algorithm is a step size, which can be constant, decreasing, or found via line search.  This algorithm is an instance of mirror descent, and thus inherits its convergence guarantees.  It will converge for any convex loss function $L$ at a $O(1 / \sqrt{t})$ rate,\footnote{That is, $L(\bmu^t) - L(\bmu^*) \in O(1 / \sqrt{t})$.} even ones that are not smooth, such as the $L_1$ loss.

We now present a related algorithm which is based on the same principles as Algorithm \ref{alg:proximal2} but has an improved $O(1/t^2)$ convergence rate for convex loss functions with Lipchitz continuous gradients.  Algorithm~\ref{alg:proximal} is based on Nesterov's accelerated dual averaging approach \cite{nesterov2009primal,xiao2010dual,vilnis2015bethe}.  The per-iteration complexity is the same as Algorithm \ref{alg:proximal2} as it requires calling the \oracle{} once, but this algorithm will converge in fewer iterations.  Algorithm \ref{alg:proximal} has the advantage of not requiring a step size to be set, but it requires knowledge of the Lipchitz constant of $ \grad L$.  For the standard $L_2$ loss with linear measurements, this is equal to the largest eigenvalue of $ \Q^T \Q $.  The derivation of this algorithm appears in the supplement.

\begin{algorithm}[tb]
    \caption{Accelerated Proximal Estimation Algorithm} \label{alg:proximal}
\begin{algorithmic}
    \STATE {\bfseries Input:} Loss function $L(\bmu)$ between $\bmu$ and $\y$
    \STATE {\bfseries Output:} Estimated data distribution $\hat{\p}_{\btheta}$
    \STATE $K = $ Lipchitz constant of $\grad L$
    \STATE $\bar{\vect{g}} = \vect{0}$
    \STATE $\vect{\nu}, \bmu = \oracle(\vect{0})$
    \FOR{$t=1, \dots, T$}
        \STATE $c = \frac{2}{t+1}$
        \STATE $\vect{\omega} = (1-c) \bmu + c \vect{\nu}$
        \STATE $\bar{\vect{g}} = (1-c) \bar{\vect{g}} + c \grad L(\vect{\omega})$
        \STATE $\btheta = \frac{-t (t+1)}{4 K} \bar{\vect{g}} $
        \STATE $\vect{\nu} = \oracle(\btheta)$
        \STATE $\bmu = (1-c) \bmu + c \vect{\nu}$
    \ENDFOR
    \STATE {\bfseries return} graphical model $\hat{\p}_{\btheta}$ with marginals $\bmu$
\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{20pt} % reset to default

%\begin{algorithm}[t]
%    \caption{Inference for Factored Queries} \label{alg:inference}
%\begin{algorithmic}
%    \STATE {\bfseries Input:} Parameters $\btheta$, factored query matrix $\Q$
%    \STATE {\bfseries Output:} Query answers $\Q\,\p_{\btheta}$
%    \STATE $\psi = \{ \exp(\btheta_C) \mid C \in \C \} \cup \{ \Q_i \mid i \in [d] \} $
%    \STATE $Z = \oracle(\btheta$)
%    \STATE {\bfseries return} $\text{VARIABLE-ELIM}(\psi, \X) / Z$
%\end{algorithmic}
%\end{algorithm}

%\textbf{Proximal Method.}\label{proximal-method}
%It is somewhat surprising that the direct problem formulation is non-convex, since the loss function is convex with respect to $\bmu$, and for every $\bmu$ we can identify the graphical model parameters $\btheta$ that give rise to those marginals (e.g., by doing learning in the graphical model).  
%
%We now present a convergent algorithm. It can be conceived as a two step process: first find an optimal $\hat{\bmu}$ by solving the convex problem $ \hat{\bmu} \in \argmin_{\bmu \in \marg} L(\bmu)$ over the marginal polytope, and then recover the model parameters $\hat{\btheta}$ that give rise to the marginals $\hat{\bmu}$. However, in practice, our algorithm for the first step will yield the model parameters ``for free''. To solve the problem over the marginal polytope, we use a variant of entropic mirror descent~\cite{beck2003mirror}, which was adapted to a similar problem by Vilnis et al.~\cite{vilnis2015bethe}.

%The procedure is shown in Algorithm~\ref{alg:proximal}; a full derivation appears in the supplement. The function $H(\bmu)$ is the Shannon entropy of the maximum-entropy distribution with marginals $\bmu$. When the graph is tree-structured there is an explicit formula for $H(\bmu)$ in terms of $\bmu$~\cite{wainwright2008graphical}. If not, $H(\bmu)$ and its gradient can be computed using a clique tree, as in our marginal oracle. \ry{Note algorithm no longer depends on $H$ so we can cut this} The algorithm accepts a sequence of non-increasing step sizes $t_1, \dots, t_K$; in our experiments we also implement a line search procedure to select step sizes. Because the problem is convex and this algorithm is an instantiation of mirror descent~\cite{beck2003mirror}, it inherits the convergence guarantees. Note that the marginals $\bmu^k$ during the $k$th iteration are obtained by calling \oracle{} on a parameter vector $\btheta^k$; thus, upon convergence to $\hat{\bmu}$, we obtain ``for free'' the parameters $\hat{\btheta}$ that lead to the optimal marginals. 
%Another nice property of this algorithm is that we recover the model parameters $\hat{\btheta}$ ``for free'' since they are used in the update equation.
%However, unlike the direct method, where we can easily apply second-order optimization algorithms like L-BFGS, mirror descent is a first-order method and may converge more slowly.
%we can't just``plug in'' the functions to compute the objective and gradient to an off-the-shelf solver, and so we don't benefit from fast second order optimization algorithms such as LBFGS. 
 
\subsection{Inference}\label{inference}

Once $\hat{\p}_{\btheta}$ has been estimated, we need algorithms to answer new queries without materializing the full contingency table representation.  This corresponds to the problem of inference in a graphical model. If the new queries only depend on $\hat{\p}_{\btheta}$ through its clique marginals $\bmu$, we can immediately answer them using \oracle{}, or by saving the final value of $\bmu$ from Algorithms~\ref{alg:proximal2} or \ref{alg:proximal}. If the new queries depend on some other marginals outside of the cliques of the graphical model, we instead use the variable elimination algorithm \cite{koller2009probabilistic} to first compute the necessary marginal, and then answer the query.  In Section \ref{sec:inference} of the supplement, we present a novel inference algorithm that is related to variable elimination but is faster for answering certain queries because it does not need to materialize full marginals if the query does not need them.  For more complicated downstream tasks, we can generate synthetic data by sampling from $\hat{\p}_{\btheta}$, although this should be avoided when possible as it introduces additional sampling error.


